Dual-Rate Force-Image Control with Model-Based Orientation Limits for Robotic Ultrasound

Robotic ultrasound couples a high-rate contact-force loop with slower, delayed image feedback, so image-guided ultrasound probe rotation can perturb contact force before the resulting image response is observed. We derive a closed-form orientation-rate limit that bounds the modeled rotation-induced estimated-force excursion over a finite horizon while accounting for disturbance rejection by the fast force loop. The limit depends on local contact stiffness, force-loop gains, a conservative rotation-to-force gain bound, the excursion budget, and the prediction horizon. We implement this model in a dual-rate controller with timestamp-based delay reconstruction and joint-torque-based force estimation, and evaluate it on a curved gelatin phantom using paired controller comparisons and component ablations. Relative to unconstrained image guidance, the proposed rate-limited controller reduced first-second root-mean-square (RMS) estimated-force error by 0.40 N while increasing cue-convergence time by 0.94 s. A fixed rate cap near the analytically predicted ceiling produced no resolvable difference in force error and converged 0.32 s faster, indicating that the principal practical value of the model is the rate-design rule rather than online prediction. Delay reconstruction had no resolvable effect at the tested latency. A single-subject popliteal scan demonstrated feasibility, although the image cue was noise-limited on heterogeneous tissue.

==> figures/architecture_diagram.tex <==
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    >=Stealth,
    font=\footnotesize,
    block/.style={
        rectangle,
        draw=black!70,
        thick,
        rounded corners=1.5pt,
        fill=white,
        align=center
    },
    plant/.style={
        rectangle,
        draw=black!80,
        very thick,
        rounded corners=2pt,
        fill=white,
        align=center
    },
    target/.style={
        rectangle,
        draw=black!70,
        thick,
        rounded corners=1.5pt,
        fill=white,
        align=center
    },
    sumcircle/.style={
        circle,
        draw=black!70,
        thick,
        inner sep=0pt,
        align=center,
        font=\small
    },
    fastline/.style={
        ->,
        >=Stealth,
        very thick,
        blue!70!black
    },
    slowline/.style={
        ->,
        >=Stealth,
        very thick,
        densely dashed,
        orange!80!black
    },
    slowblock/.style={
        draw=orange!80!black,
        densely dashed
    },
    plantline/.style={
        ->,
        >=Stealth,
        thick,
        black!75
    }
]

% ==============================================================
% MASTER ADJUSTMENT PANEL
% ==============================================================

% --------------------------------------------------------------
% FAST LOOP BOX POSITIONS
% --------------------------------------------------------------

\def\torquex{0}
\def\torquey{0}

\def\wrenchx{2.3}
\def\wrenchy{0}

\def\sumFx{4.0}
\def\sumFy{0}

\def\pidx{5.6}
\def\pidy{0}

\def\vcommandx{7.7}
\def\vcommandy{0}

\def\sumx{9.8}
\def\sumy{0}

\def\jacobianx{12.0}
\def\jacobiany{0}

\def\jointvelx{14.6}
\def\jointvely{0}

\def\plantx{17.8}
\def\planty{0}

% --------------------------------------------------------------
% FAST LOOP BOX SIZES
% --------------------------------------------------------------

\def\torquewidth{1.25cm}
\def\torqueheight{8mm}

\def\wrenchwidth{1.6cm}
\def\wrenchheight{8mm}

\def\pidwidth{1.0cm}
\def\pidheight{8mm}

\def\vcommandwidth{1.0cm}
\def\vcommandheight{8mm}

\def\sumwidth{1.55cm}
\def\sumheight{8mm}

\def\jacobianwidth{1.7cm}
\def\jacobianheight{8mm}

\def\jointvelwidth{1.0cm}
\def\jointvelheight{8mm}

\def\plantwidth{2.5cm}
\def\plantheight{15mm}

% --------------------------------------------------------------
% TARGET FORCE
% --------------------------------------------------------------

\def\fdx{4.0}
\def\fdy{1.35}

\def\fdwidth{0.9cm}
\def\fdheight{7mm}

% --------------------------------------------------------------
% SLOW LOOP BOX POSITIONS
% --------------------------------------------------------------

\def\imagex{0}
\def\imagey{-2.75}

\def\cuex{2.15}
\def\cuey{-2.75}

\def\reconstructx{4.6}
\def\reconstructy{-2.75}

\def\orientationx{6.9}
\def\orientationy{-2.75}

\def\omegax{9.2}
\def\omegay{-2.75}

\def\predictionx{11.5}
\def\predictiony{-2.75}

\def\barrierx{14.1}
\def\barriery{-2.75}

% --------------------------------------------------------------
% SLOW LOOP BOX SIZES
% --------------------------------------------------------------

\def\imagewidth{1.0cm}
\def\imageheight{8mm}

\def\cuewidth{1.0cm}
\def\cueheight{8mm}

\def\reconstructwidth{1.35cm}
\def\reconstructheight{8mm}

\def\orientationwidth{1.25cm}
\def\orientationheight{8mm}

\def\omegawidth{1.0cm}
\def\omegaheight{8mm}

\def\predictionwidth{1.55cm}
\def\predictionheight{8mm}

\def\barrierwidth{1.55cm}
\def\barrierheight{8mm}

% --------------------------------------------------------------
% THETA BUFFER
% --------------------------------------------------------------

\def\thetax{4.6}
\def\thetay{-4.8}

\def\thetawidth{1.55cm}
\def\thetaheight{8mm}

% --------------------------------------------------------------
% LOOP LABEL POSITIONS
% --------------------------------------------------------------

\def\fastlabelx{4.74}
\def\fastlabely{0.9}

\def\slowlabelx{1.88}
\def\slowlabely{-1.79}

% --------------------------------------------------------------
% BARRIER -> SUMMING JUNCTION ROUTING
% --------------------------------------------------------------

\def\barrierRouteHeight{1.15}
\def\barrierRouteX{0.25}

% --------------------------------------------------------------
% PLANT FEEDBACK HEIGHTS
% --------------------------------------------------------------

\def\plantForceFeedbackHeight{1.35}
\def\plantImageFeedbackHeight{4.74}
\def\plantThetaFeedbackHeight{4.03}

% ==============================================================
% LOOP LABELS
% ==============================================================

\node[
    anchor=west,
    text=blue!70!black,
    font=\bfseries\footnotesize
] at (\fastlabelx,\fastlabely)
{FAST LOOP: 1 kHz};

\node[
    anchor=west,
    text=orange!80!black,
    font=\bfseries\footnotesize
] at (\slowlabelx,\slowlabely)
{IMAGE LOOP: 30 Hz};

% ==============================================================
% FAST FORCE LOOP
% ==============================================================

\node[
    block,
    draw=blue!70!black,
    minimum width=\torquewidth,
    minimum height=\torqueheight,
    text width=\torquewidth
] (torque)
at (\torquex,\torquey)
{Joint\\Feedback};

\node[
    block,
    draw=blue!70!black,
    minimum width=\wrenchwidth,
    minimum height=\wrenchheight,
    text width=\wrenchwidth
] (wrench)
at (\wrenchx,\wrenchy)
{Wrench\\Estimation};

\node[
    sumcircle,
    draw=blue!70!black,
    minimum size=5.5mm
] (sumF)
at (\sumFx,\sumFy)
{$\Sigma$};

\node[
    block,
    draw=blue!70!black,
    minimum width=\pidwidth,
    minimum height=\pidheight,
    text width=19pt
] (pid)
at (\pidx,\pidy)
{Force\\PD};

\node[
    block,
    draw=blue!70!black,
    minimum width=\vcommandwidth,
    minimum height=20pt,
    text width=22pt
] (vcommand)
at (7.4,0)
{$v_n$};

% ==============================================================
% TARGET FORCE
% ==============================================================

\node[
    target,
    draw=blue!70!black,
    minimum width=\fdwidth,
    minimum height=17pt,
    text width=13pt
] (fd)
at (\fdx,\fdy)
{$F_d$};

% ==============================================================
% FAST LOOP CONNECTIONS
% ==============================================================

\draw[fastline]
    (fd.south)
    -- node[right, font=\small, near end] {$+$}
    (sumF.north);

\draw[fastline]
    (torque.east)
    -- node[above, font=\small] {$\tau_m$}
    node[below, font=\small] {$q$}
    (wrench.west);

\draw[fastline]
    (wrench.east)
    -- node[above, font=\small] {$F_n$}
    node[below, font=\small, pos=0.64] {$-$}
    (sumF.west);

\draw[fastline]
    (sumF.east)
    -- node[above, font=\small] {$e_F$}
    (pid.west);

\draw[fastline]
    (pid.east)
    -- (vcommand.west);

% ==============================================================
% COMMAND COMBINATION + PLANT
% ==============================================================

\node[
    block,
    draw=blue!70!black,
    minimum width=\sumwidth,
    minimum height=\sumheight,
    text width=\sumwidth
] (sum)
at (\sumx,\sumy)
{Compose};

\node[
    block,
    draw=blue!70!black,
    minimum width=\jacobianwidth,
    text width=52pt,
    minimum height=35pt
] (jacobian)
at (12.24,0)
{Damped Jacobian\\Pseudoinverse\\$J^{\dagger}(q)$};

\node[
    block,
    draw=blue!70!black,
    minimum width=\jointvelwidth,
    text width=39pt,
    minimum height=25pt
] (jointvel)
at (\jointvelx,\jointvely)
{Integrate\\to $q_c$};

\node[
    plant,
    minimum width=\plantwidth,
    minimum height=\plantheight,
    text width=\plantwidth
] (plant)
at (\plantx,\planty)
{Kinova Gen3\\Ultrasound Probe\\Tissue};

% scan feed (constant 5 mm/s along the traverse)
\node[
    target,
    draw=blue!70!black,
    minimum height=17pt,
    text width=13pt
] (vs)
at (\sumx,1.35)
{$v_s$};

\draw[fastline]
    (vs.south)
    -- (sum.north);

% ==============================================================
% COMMAND CONNECTIONS
% ==============================================================

\draw[fastline]
    (vcommand.east)
    -- (sum.west);

\draw[fastline]
    (sum.east)
    -- node[above, font=\small] {$v_c$}
    (jacobian.west);

\draw[fastline]
    (jacobian.east)
    -- node[above, font=\small] {$\dot q_c$}
    (jointvel.west);

\draw[fastline]
    (jointvel.east)
    -- node[above, font=\small] {$q_c$}
    (plant.west);

% ==============================================================
% IMAGE / ORIENTATION LOOP
% ==============================================================

\node[
    block,
    slowblock,
    minimum width=\imagewidth,
    minimum height=\imageheight,
    text width=\imagewidth
] (image)
at (\imagex,\imagey)
{B-mode\\Image};

\node[
    block,
    slowblock,
    minimum width=\cuewidth,
    text width=39pt
] (cue)
at (\cuex,\cuey)
{Cue\\Estimation};

\node[
    block,
    draw=blue!70!black,
    minimum width=\reconstructwidth,
    minimum height=\reconstructheight,
    text width=54pt
] (reconstruct)
at (\reconstructx,\reconstructy)
{Filter and\\Delay\\Reconstruction};

\node[
    block,
    draw=blue!70!black,
    minimum width=\orientationwidth,
    text width=43pt
] (orientation)
at (7.07,-2.75)
{Orientation\\Law};

\node[
    block,
    draw=blue!70!black,
    minimum width=\omegawidth,
    minimum height=21pt,
    text width=14pt
] (omega)
at (\omegax,\omegay)
{$\omega$};

\node[
    block,
    slowblock,
    minimum width=\predictionwidth,
    minimum height=\predictionheight,
    text width=\predictionwidth
] (prediction)
at (\predictionx,\predictiony)
{Predictive\\Force Model};

\node[
    block,
    slowblock,
    minimum width=\barrierwidth,
    minimum height=\barrierheight,
    text width=\barrierwidth
] (barrier)
at (\barrierx,\barriery)
{Log-Barrier\\Rate Scaling\\$s\in[0,1]$};

% ==============================================================
% SLOW LOOP CONNECTIONS
% ==============================================================

\draw[slowline]
    (image.east)
    -- (cue.west);

\draw[slowline]
    (cue.east)
    -- node[above, font=\small] {$I$}
    node[below, font=\small] {$t^c$}
    (reconstruct.west);

\draw[fastline]
    (reconstruct.east)
    -- node[above, font=\small] {$\hat I$}
    (orientation.west);

\draw[fastline]
    (orientation.east)
    -- (omega.west);

\draw[slowline]
    (omega.east)
    -- (prediction.west);

\draw[slowline]
    (prediction.east)
    -- node[above, font=\small] {$u(s)$}
    (barrier.west);

% ==============================================================
% BARRIER -> COMMAND SUM
% ==============================================================

\draw[fastline]
    (barrier.north)
    -- ++(0,0.59)
    -| node[font=\small, near start, above] {$s\omega$}
    (sum.south);

% ==============================================================
% THETA BUFFER
% ==============================================================

\node[
    block,
    draw=blue!70!black,
    minimum width=\thetawidth,
    minimum height=\thetaheight,
    text width=\thetawidth
] (theta)
at (4.59,-4.2)
{$\theta$\\Buffer};

% ==============================================================
% THETA -> RECONSTRUCTION
% ==============================================================

\draw[fastline]
    (theta.north)
    -- node[right, font=\small] {$\theta(t)$}
    (reconstruct.south);

% ==============================================================
% PLANT FEEDBACK
% ==============================================================

\draw[plantline]
    (plant.north)
    -- ++(0,1.23)
    -| (torque.north);

\draw[plantline]
    (plant.south)
    -- ++(0,-4.23)
    -| (image.south);

\draw[
    plantline,
    ->
]
    (plant.south)
    -- ++(0,-\plantThetaFeedbackHeight)
    |- node[pos=0.97, above, font=\small] {$q$}
    (theta.east);

% ==============================================================
% END DIAGRAM
% ==============================================================

\end{tikzpicture}%
}

==> sections_v1/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Brightness mode (B-mode) ultrasound provides real-time, radiation-free imaging with comparatively low cost, but its image quality is strongly coupled to how the probe interacts with the tissue. During manual scanning, a sonographer continuously
coordinates probe position and orientation with contact force while responding to local surface geometry, tissue compliance, and the observed ultrasound image. Robotic ultrasound, therefore, presents a coupled sensing-and-control problem rather than a conventional trajectory-following task. Existing reviews accordingly identify scanning-path generation, probe-tissue force regulation, and image-quality or orientation optimization as central components of autonomous robotic ultrasound systems \cite{li2021overview,haxthausen2021,salcudean2022,jiang2023review}. More recent surveys note two remaining limitations that are particularly relevant from a control perspective: interaction wrench components associated with probe orientation are often simplified, and real-time ultrasound feedback remains less commonly integrated into online scan optimization \cite{bi2024,munir2025,han2025clinical}. These limitations motivate control architectures in which the probe-tissue dynamics, cross-coupling between controlled variables, and heterogeneous sensing rates are treated explicitly. 

Early image-guided robotic ultrasound demonstrated that features extracted directly from ultrasound images can close the robot-positioning loop \cite{abolmaesumi2002}. Subsequent visual-servoing approaches optimized ultrasound confidence measures to improve acoustic coupling and probe orientation \cite{chatelain2015}. In parallel, interaction-force information has been exploited for estimating the local surface normal and regulating probe orientation \cite{jiang2020normal,jiang2021force,ma2022asee}. More recent explicit force-control strategies directly regulate contact forces and moments to achieve responsive probe - tissue interaction under heterogeneous and dynamic conditions \cite{piedra2026}. Ultrasound feedback has also enabled autonomous entering and alignment of tubular structures \cite{jiang2022tubular}, while image-quality estimated have been used to adapt the commanded contact force rather than maintaining a fixed force across different imaging conditions \cite{akbari2021,zakeri2025}. Collectively, these studies establish that image and force sensing provide complementary information. Consequently, simply combining the two feedback modalities is no longer, by itself, sufficient to contribute to control. 

Learning-based approaches have further expanded the achievable level of autonomy. Deep reinforcement learning has been used to navigate toward anatomical targets from ultrasound observations \cite{hase2020}; reinforcement learning policies have combined visual scene perception with compliant force control for scanning moving, markerless targets \cite{ning2021rl}; and inverse reinforcement learning has transferred active-compliance behavior to uncertain soft environments \cite{ning2024irl}. Constraint-aware policy optimization explicitly incorporates interaction-force limits during policy learning \cite{duan2025safe}, while recent large-scale imitation learning has demonstrated substantial generalization across an autonomous carotid-ultrasound workflow \cite{jiang2025ultrabot}. These developments demonstrate the potential of learning for perception, decision making, and reference generation. At the same time, recent reviews emphasize limitations associated with medical-data availability, domain variation, and insufficient incorporation of physical knowledge \cite{bi2024,yip2023}. For contact-rich medical robotics, this suggests a useful separation of roles: learned perception can provide task-relevant image information, whereas the high-bandwidth interaction loop should retain sufficient physical structure to support constraint enforcement, robustness analysis, and failure detection. 

A control issue that is less explicitly addressed in this literature is the multirate dynamic coupling between force regulation and image-guided probe correction. Robot state and wrench measurements can be updated at high rates, whereas B-mode images are acquired, transferred, and processed at substantially lower rates and with non-negligible latency. This mismatch has already appeared in practical robotic ultrasound implementations; for example, image-based force adjustment has been implemented with a slower image-quality loop than the underlying robot-control loop \cite{akbari2021}. The difficulty is more fundamental than asynchronous sensing alone. An orientation correction computed from an image changes probe indentation, the contact moment, and consequently the normal force before a new image measurement becomes available. Conversely, a fast force regulator reacts to the normal displacement induced by the orientation update and can partially oppose the intended image-based correction. Tissue stiffness, local curvature, surface motion, and uncertainty in image sensitivity further modify this bidirectional interaction. Recent dual-loop approaches have demonstrated image-dependent force adaptation and robust contact-force tracking \cite{zakeri2025}, while explicit force/moment regulation improves dynamic interaction performance \cite{piedra2026}. In addition, Li et al. \cite{li2026trajectory} explicitly incorporate trajectory-dependent feedforward and delay compensation for dynamic contact-force tracking, and Qian et al. \cite{qian2026symmetry} combine image guidance with biomechanics-informed force estimation/control. However, these advances do not directly formulate the image-guided orientation loop and the high-rate force loop as an identified, delayed multirate system whose cross-coupling can be predicted and incorporated into controller design. 


This paper addresses this control gap through a model-informed dual-rate framework for dynamic robotic ultrasound interaction. Rather than pursuing end-to-end autonomous diagnosis, we focus on a narrower control objective: coordinating normal interaction force with an ultrasound-derived orientation feature while explicitly accounting for probe-tissue coupling, image latency, model uncertainty, and operational constraints. A local input-output model is identified from bounded excitation experiments and lifted to the image-update timescale, allowing the slower image-guided controller to predict the force consequences of orientation corrections while a faster inner loop regulates probe-tissue contact. This structure preserves high-rate interaction control while using ultrasound information where it is most informative. The main contributions are:

\begin{enumerate}
    \item a physically interpretable operational-space interaction model and bounded identification procedure that characterize normal compliance, orientation-to-force coupling, image-feature sensitivity, transport delay, and model uncertainty using independent validation trials;

    \item a dual-rate control architecture that combines high-rate disturbance-compensated normal-force regulation with a slower, delay-aware and constraint-aware image-guided update based on the identified lifted model, thereby accounting explicitly for the interaction between orientation correction and contact force;

    \item sufficient small-gain and feasibility conditions for practical boundedness of the coupled closed-loop system, together with an independent contact-safety supervisor whose operation does not rely on ultrasound-image inference; and

    \item repeated hardware experiments on tissue-mimicking phantom and human tissue conditions, including controlled ablations that isolate the contributions of image feedback, force-orientation coupling compensation, and explicit delay handling relative to defined baseline controllers.
\end{enumerate}

The resulting framework is intended to bridge high-bandwidth interaction control and lower-rate image-guided adaptation without requiring either loop to be collapsed into a single-rate controller or an end-to-end learned policy.


==> sections_v1/02_system_problem.tex <==
\section{System and Problem Formulation}
\label{sec:system}

\subsection{Robotic Ultrasound and Operational-Space Dynamics}

The experimental platform consists of a Kinova manipulator, an ultrasound transducer rigidly mounted to the end effector, a six-axis force/torque sensor, and a B-mode ultrasound system. The robot model, probe specifications, acquisition interface, probe-mount geometry, and computing hardware are reported in Section~{V} after hardware verification. Robot states and wrench measurements are sampled at $f_f=1000$ Hz, whereas B-mode images are acquired at $f_I=25$ Hz. The image pipeline introduces an experimentally measured acquisition-to-processing delay of $\tau_I=20-
30$ ms with bounded jitter. All robot, wrench, and ultrasound data are timestamped using a common clock.

Let $\vect q\in\mathbb{R}^{n_q}$ denote the joint configuration and $J(\vect q)$ the end-effector Jacobian. The rigid-body manipulator dynamics are written as
\begin{equation}
 M(\vect q)\ddot{\vect q}
 +C(\vect q,\dot{\vect q})\dot{\vect q}
 +\vect g(\vect q)
 =
 \vect\tau
 +J^{\mathsf T}(\vect q)\,{}^{B}\vect h_c,
 \label{eq:robot_dynamics}
\end{equation}
where $\vect\tau$ is the commanded joint torque and $\,{}^{B}\vect h_c=[{}^{B}\vect F_c^{\mathsf T},{}^{B}\vect\mu_c^{\mathsf T}]^{\mathsf T}$ is the external contact wrench exerted by the environment on the robot, expressed in the base frame.

The controller is implemented through an operational-space interface that separates probe-normal translation from tangential and rotational motion \cite{khatib1987}. Let $\{B\}$, $\{E\}$, $\{S\}$, and $\{P\}$ denote the robot-base, end-effector, wrench-sensor, and probe frames, respectively. The measured sensor wrench is transformed to the probe frame and compensated according to
\begin{equation}
 {}^{P}\vect h_c
 =
 {}^{P}\!X_{S}^{*}\,{}^{S}\vect h_m
 -{}^{P}\vect h_g(\vect q)
 -{}^{P}\vect b_h,
 \label{eq:wrench_transform}
\end{equation}
where ${}^{P}\!X_{S}^{*}$ is the calibrated wrench transformation from $\{S\}$ to $\{P\}$, ${}^{P}\vect h_g$ is the orientation-dependent payload/gravity wrench of the probe assembly, and ${}^{P}\vect b_h$ is the calibrated sensor bias. Recomputing the gravity term during probe rotation prevents orientation-dependent payload effects from being misinterpreted as probe--tissue coupling.

\subsection{Local Contact Geometry and Multirate Measurements}

Let $\vect e_n=[0\;0\;1]^{\mathsf T}$ denote the probe-normal axis in $\{P\}$, chosen to point from the probe face into the tissue. Its base-frame representation is
\begin{equation}
 {}^{B}\vect n(\vect\theta)
 ={}^{B}R_{P}(\vect\theta)\vect e_n,
\end{equation}
where $\vect\theta\in\mathbb{R}^{n_\theta}$ contains the one or two controlled probe-tilt angles. For a probe-face reference point ${}^{B}\vect p_e$ and the corresponding undeformed local surface point ${}^{B}\vect p_s$, define the signed indentation
\begin{equation}
 \delta
 =
 {}^{B}\vect n^{\mathsf T}(\vect\theta)
 \left({}^{B}\vect p_e-{}^{B}\vect p_s\right),
 \label{eq:indentation}
\end{equation}
so that $\delta>0$ corresponds to compression into the tissue.

Because ${}^{B}\vect h_c$ in \eqref{eq:robot_dynamics} is the wrench exerted by the environment on the robot, the positive compressive normal-force magnitude is defined as
\begin{equation}
 F_n
 =
 -{}^{B}\vect n^{\mathsf T}{}^{B}\vect F_c,
 \qquad
 \vect\mu_t
 =
 \left(I-{}^{B}\vect n{}^{B}\vect n^{\mathsf T}\right){}^{B}\vect\mu_c.
 \label{eq:normal_force}
\end{equation}
The minus sign in $F_n$ follows from the chosen convention: during compression, the tissue reaction force on the probe is opposite to the probe-normal direction. In implementation, the measured wrench is transformed to the common control frame before evaluating \eqref{eq:normal_force}. The tangential moment is retained as an independent indicator of departure from the local contact regime.
The fast force loop executes at
\begin{equation}
 t_k=kT_f,
 \qquad
 T_f=f_f^{-1}.
\end{equation}
For the nominal dual-rate formulation, let
\begin{equation}
 T_I=mT_f,
 \qquad
 m\in\mathbb{N},
\end{equation}
where $T_I$ is the nominal image period. The $j$th image is captured at
\begin{equation}
 t_j^c=jT_I+\epsilon_j^c
\end{equation}
and becomes available after processing at
\begin{equation}
 t_j^a=t_j^c+\tau_j,
 \label{eq:image_timing}
\end{equation}
where $\epsilon_j^c$ is bounded acquisition jitter and $\tau_j$ is the acquisition-to-processing latency. The slow controller is updated at nominal times $t_j^s=jT_I$ using the most recent valid image available at that instant. Define
\begin{equation}
 \ell_j
 =
 \max\{\ell: t_\ell^a\leq t_j^s\},
 \qquad
 d_j=j-\ell_j,
 \label{eq:image_age}
\end{equation}
where $d_j$ is the image age in frame intervals. The admissible delay condition is $0\leq d_j\leq \bar d_I$; larger image age or missing valid frames triggers supervisory logic.

Let $\vect s_I(I_j)\in\mathbb{R}^{n_I}$ denote a deterministic image feature associated with the image capture time $t_j^c$. The force and image errors are
\begin{align}
 e_F(k)
 &=F_n(k)-F_d(k),
 \label{eq:force_error}\\
 \vect e_I(j)
 &=\vect s_I(I_j)-\vect s_{I,d}.
 \label{eq:image_error}
\end{align}
To distinguish an orientation command from an orientation increment, define
\begin{equation}
 \vect\vartheta_j
 =
 \vect\theta_{d,j}-\vect\theta_0,
 \qquad
 \Delta\vect\theta_j
 =
 \vect\vartheta_j-\vect\vartheta_{j-1},
 \label{eq:tilt_notation}
\end{equation}
where $\vect\theta_0$ is the nominal probe orientation. Thus, $\vect\vartheta_j$ is the held orientation deviation during interval $j$, whereas $\Delta\vect\theta_j$ is the slow controller update. The hard operating limits are
\begin{equation}
\begin{aligned}
 F_{\min}
 &\leq F_n(k)\leq F_{\max},\\
 \vect\theta_{d,j}
 &\in\Theta,\\
 \Delta\vect\theta_j
 &\in\Delta\Theta,\\
 \norm{\vect\mu_t(k)}
 &\leq\mu_{\max}.
\end{aligned}
\label{eq:constraints}
\end{equation}

\subsection{Control Objective and Local Assumptions}

The controller is designed for a bounded neighborhood of a nominal probe-tissue contact condition. The following assumptions define the local operating region.

\textit{(A1):} Probe-tissue contact is maintained, and the local tissue surface is continuously differentiable within the controlled patch. \textit{(A2):} Local contact stiffness, damping, surface velocity, and unmodeled disturbances are bounded within each accepted contact condition. \textit{(A3):} Image acquisition jitter and processing delay are bounded, with $d_j\leq\bar d_I$. Exceeding this bound, repeated frame loss, or invalid image quality triggers the supervisor. \textit{(A4):} Within the image-controller trust region, the selected image feature is locally Lipschitz in force and orientation, and its orientation-sensitivity matrix has full column rank for the controlled tilt axes. \textit{(A5):} The underlying robot motion interface is internally stable over the commanded operating range. After the input coordinate is selected, the identified normal-force channel has a known control direction, i.e., $b\geq b_{\min}>0$ for all accepted models.

Under A1--A5, the control objective is to design the fast normal command $u_{n,k}$, the slow orientation increment $\Delta\vect\theta_j$, and an independent supervisory policy such that: (i) the force error $e_F(k)$ and image error $\vect e_I(j)$ remain practically bounded and are driven toward neighborhoods of their desired values; (ii) multirate force--orientation coupling and delayed image feedback are explicitly incorporated into the control design; and (iii) the hard force, pose, rate, and supervisory moment limits in \eqref{eq:constraints} are respected whenever the robust admissible-control sets remain nonempty.

Violations of the local model assumptions are treated as supervisory events rather than as nominal closed-loop convergence failures. In particular, contact loss, excessive moment, stale image measurements, image-feature degeneracy, workspace violations, sensor faults, and communication faults are handled independently of image inference.

==> sections_v1/03_model_identification.tex <==
\section{Modeling and System Identification}
\label{sec:model}

\subsection{Local Force--Pose Interaction Model}

Within a bounded contact patch, the normal probe--tissue interaction is approximated by a Kelvin--Voigt relation,
\begin{equation}
 F_n
 =
 k(\rho)\delta
 +c(\rho)\dot\delta
 +b_F
 +\eta_F,
 \label{eq:kelvin_voigt}
\end{equation}
where $k(\rho)>0$ and $c(\rho)\geq0$ are local effective stiffness and damping coefficients, $b_F$ is a residual force offset, $\eta_F$ represents unmodeled interaction effects, and $\rho$ indexes the local contact condition.

Linearizing the indentation about a nominal operating point $(\vect p_{e,0},\vect\theta_0)$ gives
\begin{equation}
 \delta
 \simeq
 \delta_0
 +\Delta p_n
 +\vect r_\theta^{\mathsf T}\vect\vartheta
 +d_s,
 \label{eq:contact_linearization}
\end{equation}
where $\Delta p_n$ is the probe displacement along the positive compression direction, $\vect\vartheta$ is the local orientation deviation defined in \eqref{eq:tilt_notation}, $\vect r_\theta$ maps small probe rotations into changes in effective indentation, and $d_s$ is defined positive when surface motion increases indentation. Equation~\eqref{eq:contact_linearization} is a local input--output approximation, not a global soft tissue model.

After discretization and inclusion of the closed inner robot-servo dynamics, define
\begin{equation}
 \vect x_k
 =
 \begin{bmatrix}
 e_F(k) & \Delta p_n(k) & \dot{\Delta p}_n(k)
 \end{bmatrix}^{\mathsf T}.
\end{equation}
A local scheduled fast-rate model is
\begin{align}
 \vect x_{k+1}
 ={}&
 A(\rho_k)\vect x_k
 +B_n(\rho_k)u_{n,k}
 +B_\vartheta(\rho_k)\vect\vartheta_{j(k)}
 \nonumber\\
 &+
 E(\rho_k)\vect d_k
 +\vect w_k,
 \label{eq:fast_model}\\
 y_{F,k}
 ={}&
 C_F\vect x_k+v_{F,k},
 \label{eq:force_output_model}
\end{align}
where $j(k)=\lfloor k/m\rfloor$, $\vect d_k$ contains bounded exogenous terms such as surface motion and force-reference variation, and $\vect w_k$ and $v_{F,k}$ denote bounded model and sensing errors. The model order is kept deliberately low and is increased only when complete held-out trials show a material improvement in multi-step prediction.

\subsection{Image Feature Dynamics and Local Sensitivity}

For probe-normal alignment, an acoustic-confidence map $Q(I_j)$ is partitioned into left/right regions and, when the second tilt axis is observable, upper/lower regions. A representative two-axis image error is
\begin{equation}
 \vect e_I(j)
 =
 \begin{bmatrix}
 \overline Q_L-\overline Q_R\\
 \overline Q_U-\overline Q_D
 \end{bmatrix}
 -\vect s_{I,d},
 \label{eq:image_feature}
\end{equation}
where $\overline Q_\bullet$ denotes the mean confidence in the corresponding region. For a single controlled tilt axis, only the corresponding observable component is retained. Mean confidence, contrast-to-noise ratio, entropy, and other global image-quality metrics are treated as evaluation quantities unless they are explicitly included in the control feature.

Small bounded orientation perturbations around $(\vect\theta_0,F_{d,0})$ are used to identify the slow-rate image dynamics
\begin{equation}
 \vect e_I(j+1)
 =
 A_I\vect e_I(j)
 +L_\theta\Delta\vect\theta_j
 +L_F\bar e_F(j)
 +\vect v_{I,j},
 \label{eq:image_model}
\end{equation}
where
\begin{equation}
 \bar e_F(j)
 =
 \frac{1}{m}
 \sum_{r=0}^{m-1}e_F(jm+r)
 \label{eq:mean_force_error}
\end{equation}
is the mean force error over image interval $j$. The singular values of $L_\theta$ quantify local orientation observability. Controller operation is restricted to a trust region in which the relevant minimum singular value remains above a prescribed threshold and the held-out linearization residual remains within the accepted bound.

If a deterministic image feature is experimentally insufficient, it may be replaced by a frozen estimator $q_\phi(I)$. Any learned estimator is trained with phantom- or subject-level separation, evaluated on held-out domains, timed on the deployment computer, frozen before controller comparison, and excluded from the independent hard-safety path.

\subsection{Fast-Rate Lifting and Within-Interval Force Prediction}

For a fixed accepted local model over one image interval, write $A=A(\rho_j)$, $B_n=B_n(\rho_j)$, $B_\vartheta=B_\vartheta(\rho_j)$, and $E=E(\rho_j)$. Define the slow-indexed fast state
\begin{equation}
 \vect x_j^s=\vect x_{jm}
\end{equation}
and stack the fast normal commands as
\begin{equation}
 \vect U_{n,j}
 =
 \operatorname{col}
 \left(u_{n,jm},\ldots,u_{n,(j+1)m-1}\right).
\end{equation}
Iterating \eqref{eq:fast_model} over $m$ fast samples gives
\begin{align}
 \vect x_{j+1}^s
 ={}&
 A^m\vect x_j^s
 +\mathcal B_n\vect U_{n,j}
 +\mathcal B_\vartheta\vect\vartheta_j
 \nonumber\\
 &+
 \mathcal E_m\vect D_j
 +\vect W_j,
 \label{eq:lifted_model}
\end{align}
where
\begin{align}
 \mathcal B_n
 &=
 \begin{bmatrix}
 A^{m-1}B_n & A^{m-2}B_n & \cdots & B_n
 \end{bmatrix},\\
 \mathcal B_\vartheta
 &=
 \sum_{r=0}^{m-1}A^{m-1-r}B_\vartheta.
 \label{eq:lifted_matrices}
\end{align}
The vectors $\vect D_j$ and $\vect W_j$ contain the corresponding lifted disturbances and model errors.

Because the slow optimizer must protect force constraints at the fast sampling rate, endpoint prediction alone is insufficient. Define the stacked within-interval force-error trajectory
\begin{equation}
 \vect e_{F,j}^{\mathrm{stk}}
 =
 \operatorname{col}
 \left(e_F(jm+1),\ldots,e_F((j+1)m)\right).
\end{equation}
Using \eqref{eq:fast_model}, this trajectory can be written in standard lifted form as
\begin{equation}
 \vect e_{F,j}^{\mathrm{stk}}
 =
 \mathcal O_F\vect x_j^s
 +\mathcal T_{Fn}\vect U_{n,j}
 +\mathcal T_{F\vartheta}\vect\vartheta_j
 +\mathcal T_{Fd}\vect D_j
 +\vect V_{F,j},
 \label{eq:stacked_force_prediction}
\end{equation}
where
\begin{equation}
 \mathcal O_F
 =
 \operatorname{col}
 \left(C_FA,C_FA^2,\ldots,C_FA^m\right),
\end{equation}
and $\mathcal T_{Fn}$, $\mathcal T_{F\vartheta}$, and $\mathcal T_{Fd}$ are the corresponding lower block-Toeplitz matrices. Equation~\eqref{eq:stacked_force_prediction} is the quantity used later to impose force limits at every fast sample inside the slow prediction horizon.

\subsection{Timestamped Image Delay and State Reconstruction}

The image delay is represented as a delayed measurement rather than as an artificial plant delay. At slow update $j$, the most recent available image has index $\ell_j$ defined in \eqref{eq:image_age}, so the available image measurement is
\begin{equation}
 \vect y_{I,j}
 =
 \vect e_I(\ell_j)
 +\vect\nu_{I,j},
 \qquad
 d_j=j-\ell_j\leq\bar d_I.
 \label{eq:delayed_image_measurement}
\end{equation}
Because all orientation commands and fast force measurements applied between $\ell_j$ and $j$ are known, the current image-feature estimate can be propagated from the delayed measurement using \eqref{eq:image_model}:
\begin{align}
 \widehat{\vect e}_{I,j|j}
 ={}&
 A_I^{d_j}\vect y_{I,j}
 \nonumber\\
 &+
 \sum_{r=0}^{d_j-1}
 A_I^{d_j-1-r}
 \left(
 L_\theta\Delta\vect\theta_{\ell_j+r}
 +L_F\bar e_F(\ell_j+r)
 \right).
 \label{eq:image_state_reconstruction}
\end{align}
For $d_j=0$, \eqref{eq:image_state_reconstruction} reduces to the current image measurement. The accumulated effect of image noise, model mismatch, acquisition jitter, and sub-frame timing mismatch is bounded from validation data and included in the image-side uncertainty margin. If $d_j>\bar d_I$ or the image validity test fails, no new image-based orientation update is issued.

\subsection{Identification and Validation Protocol}

Before dynamic identification, the wrench bias, probe payload, probe-frame transform, and gravity compensation are calibrated. The robot then establishes a nominal contact operating point of \tbd{$10~\mathrm{N}$} on the tissue-mimicking phantom. Bounded multisine, chirp, or pseudo-random binary excitations are applied independently along the normal direction and each controlled tilt axis, followed by a bounded combined excitation to identify cross-coupling. Excitation amplitudes and spectra are chosen to cover the intended force-control bandwidth and expected surface-motion band while satisfying the predetermined force, moment, pose, and velocity limits.

Image latency is estimated independently from the dynamic coefficients so that transport delay is not spuriously absorbed into the fitted interaction parameters. Because the force and image models evolve at different rates, their parameters are estimated from separate regressions. For subsystem $\ell\in\{F,I\}$, let $\vect\phi_{\ell,r}$ denote the corresponding regression vector and $\vect y_{\ell,r+1}$ the measured next-step output. The estimate is
For each $\ell\in\{F,I\}$, the estimate is
\begin{equation}
\begin{aligned}
 \widehat\Theta_\ell
 =\arg\min_{\Theta_\ell}\;&
 \sum_{r\in\mathcal T_\ell}
 \norm{
 \vect y_{\ell,r+1}-\Theta_\ell\vect\phi_{\ell,r}
 }_{W_\ell}^{2}\\
 &+\lambda_\ell\norm{\Theta_\ell}_{F}^{2}.
\end{aligned}
 \label{eq:id_objective}
\end{equation}
The fast-model training set $\mathcal T_F$ contains fast-rate samples, whereas $\mathcal T_I$ contains complete image intervals together with timestamp-aligned force summaries.

Training and validation are separated at the level of complete trials and contact locations rather than adjacent time samples. Candidate models are evaluated using normalized multi-step prediction error, residual bias and autocorrelation, numerical stability, parameter variation across contact sites, and prediction under disturbances not used for fitting. Model order and scheduling complexity are increased only when improvement persists on complete held-out trials.

For control implementation, the accepted parametric uncertainty is represented by a finite model bank
\begin{equation}
 \mathcal P
 =
 \left\{p^{(1)},\ldots,p^{(N_p)}\right\},
 \label{eq:model_bank}
\end{equation}
constructed from accepted local fits and other explicitly evaluated uncertainty scenarios. Additive held-out prediction errors are bounded separately by compact residual sets and are enlarged, when necessary, to cover interpolation between the retained scenarios over the certified trust region. Thus, robustness claims are made with respect to the finite scenario bank plus the stated residual bounds, not automatically with respect to the entire convex hull of the original identified parameters. This finite representation is important computationally: when each scenario produces affine state/output predictions and the constraints are linear, the robust slow optimization remains a quadratic program. If a continuous uncertainty set is retained instead, the corresponding exact robust counterpart need not remain a QP and must be reformulated accordingly.

\begin{figure}[t]
    \centering
    \fbox{\parbox[c][1.04in][c]{0.94\columnwidth}{\centering
    \tbd{Fig. 2: bounded identification inputs; measured and predicted force/image features; residual autocorrelation; held-out prediction.}}}
    \caption{Identification and validation workflow. The final figure will report excitation spectra, retained model order, measured image delay, training/validation partition, uncertainty construction, representative held-out predictions, and residual diagnostics.}
    \label{fig:id_placeholder}
\end{figure}


==> sections_v1/04_control.tex <==
\section{Dual-Rate Constrained Control}
\label{sec:control}

\subsection{Fast Normal-Force Regulation}

The existing normal-force controller without image-informed coupling compensation is retained as baseline B1. For controller analysis, the identified normal-force channel is reduced locally to
\begin{equation}
 e_F(k+1)
 =
 a e_F(k)
 +b u_{n,k}
 +\vect g^{\mathsf T}\vect\vartheta_{j(k)}
 +d_k,
 \label{eq:scalar_force_model}
\end{equation}
where $b\geq b_{\min}>0$ by the input-sign convention in A5, $\vect\vartheta_{j(k)}$ is the held orientation deviation, and $d_k$ collects bounded surface motion, force-reference variation, and residual model mismatch.

The proposed nominal fast controller is
\begin{align}
 u_{n,k}^{0}
 ={}&
 -K_p e_F(k)
 -K_i\xi_k
 -\widehat b^{-1}\widehat{\vect g}^{\mathsf T}\vect\vartheta_{j(k)}
 \nonumber\\
 &+
 u_{{\rm ff},k}
 -\widehat b^{-1}\widehat d_k,
 \label{eq:fast_controller}
\end{align}
where $\widehat b$ and $\widehat{\vect g}$ are the nominal identified input and orientation-coupling coefficients, $u_{{\rm ff},k}$ is optional measured/reference feedforward expressed in command units, and $\widehat d_k$ is a low-bandwidth estimate of the additive disturbance in \eqref{eq:scalar_force_model}. Using identified nominal coefficients rather than the unknown true coefficients makes any cancellation error explicit and places it in the robust residual term.

The integral state is updated using the finally applied fast command $u_{n,k}$,
\begin{equation}
 \xi_{k+1}
 =
 \xi_k
 +T_f e_F(k)
 +k_{\rm aw}\left(u_{n,k}-u_{n,k}^{0}\right),
 \label{eq:antiwindup}
\end{equation}
so that actuator limiting or safety-filter intervention is reflected in the anti-windup path.

The disturbance estimate is updated from the one-step model innovation,
\begin{align}
 \widehat d_{k+1}
 ={}&
 (1-\ell)\widehat d_k
 \nonumber\\
 &+
 \ell\left[
 e_F(k+1)
 -\widehat a e_F(k)
 -\widehat b u_{n,k}
 -\widehat{\vect g}^{\mathsf T}\vect\vartheta_{j(k)}
 \right],
 \label{eq:disturbance_observer}
\end{align}
with $0<\ell<1$. Under the exact nominal scalar model, the bracketed term equals $d_k$. If $\widetilde d_k=d_k-\widehat d_k$ and $|d_{k+1}-d_k|\leq\bar\Delta_d$, then
\begin{equation}
 |\widetilde d_k|
 \leq
 (1-\ell)^k|\widetilde d_0|
 +\frac{\bar\Delta_d}{\ell},
 \label{eq:disturbance_error_bound}
\end{equation}
while model-parameter mismatch adds to the same residual bound. Integrator and disturbance-estimator states are frozen or reinitialized after contact loss, invalid wrench sensing, emergency retraction, or another supervisory fault.

\subsection{Closed-Loop Lifted Predictor}

The slow image controller changes probe orientation but does not independently optimize the $m$ fast normal commands. Therefore, treating $\vect U_{n,j}$ in \eqref{eq:lifted_model} as a free slow-level decision would be inconsistent with the implemented architecture. Instead, the nominal fast control law \eqref{eq:fast_controller}--\eqref{eq:antiwindup} is substituted into the identified fast model before lifting.

For each model $p^{(s)}\in\mathcal P$, define a fast closed-loop prediction state $\vect\chi_k^{(s)}$ that contains the identified force-model state together with the PI and disturbance-estimator states required for prediction. In the planned operating region, the safety filter is assumed inactive inside the slow predictor; its intervention is treated as a measured deviation and has priority over the performance controller. The resulting nominal fast prediction is linear-affine in $\vect\chi_k^{(s)}$ and the held orientation command. Lifting it over one image interval and augmenting with the image state and orientation command gives
\begin{equation}
 \vect z_{j+1}^{(s)}
 =
 A_L^{(s)}\vect z_j^{(s)}
 +B_L^{(s)}\Delta\vect\theta_j
 +E_L^{(s)}\vect d_j,
 \label{eq:closed_loop_lifted}
\end{equation}
where $\vect z_j^{(s)}$ includes the slow-sampled fast-loop state, the current reconstructed image-feature state, and the previous held orientation command. The corresponding stacked fast-rate force trajectory over interval $j$ is
\begin{equation}
 \vect F_{n,j}^{(s)}
 =
 C_{F,L}^{(s)}\vect z_j^{(s)}
 +D_{F,L}^{(s)}\Delta\vect\theta_j
 +G_{F,L}^{(s)}\vect d_j
 +\vect F_{d,j},
 \label{eq:closed_loop_force_stack}
\end{equation}
where $\vect F_{d,j}$ stacks the force reference over the same $m$ fast samples. The matrices in \eqref{eq:closed_loop_lifted} and \eqref{eq:closed_loop_force_stack} are obtained by substituting the fast controller into \eqref{eq:fast_model} and \eqref{eq:stacked_force_prediction}, respectively. Thus, a candidate orientation update is evaluated together with the force response predicted to occur at each fast sample. The predicted mean force error used below is
\begin{equation}
 \widehat{\bar e}_{F,j}^{(s)}
 =
 \frac{1}{m}\vect 1_m^{\mathsf T}
 \left(\vect F_{n,j}^{(s)}-\vect F_{d,j}\right).
 \label{eq:predicted_mean_force_error}
\end{equation}

At slow time $j$, the reconstructed current image state $\widehat{\vect e}_{I,j|j}$ from \eqref{eq:image_state_reconstruction} is used to initialize $\vect z_j^{(s)}$. The reconstruction error associated with delayed images is included in the additive uncertainty margin.

\subsection{Slow Image-Guided Orientation Program}

Over a horizon of $N$ image intervals, define
\begin{equation}
 \Delta\vect\Theta_j
 =
 \operatorname{col}
 \left(
 \Delta\vect\theta_{j|j},\ldots,
 \Delta\vect\theta_{j+N-1|j}
 \right).
\end{equation}
For each uncertainty scenario $s=1,\ldots,N_p$, predictions satisfy \eqref{eq:closed_loop_lifted}. The held orientation sequence is reconstructed from
\begin{equation}
 \vect\vartheta_{j-1|j}=\vect\vartheta_{j-1},
 \qquad
 \vect\vartheta_{j+r|j}
 =
 \vect\vartheta_{j+r-1|j}
 +\Delta\vect\theta_{j+r|j}.
 \label{eq:orientation_recursion}
\end{equation}
For scenario $s$, define the quadratic stage-horizon cost
\begin{align}
 J_j^{(s)}
 =\sum_{r=0}^{N-1}\Big(&
 \norm{\widehat{\vect e}_{I,j+r|j}^{(s)}}_{W_I}^{2}
 +w_F\left|\widehat{\bar e}_{F,j+r|j}^{(s)}\right|^2
 \nonumber\\
 &+\norm{\Delta\vect\theta_{j+r|j}}_{R}^{2}\Big).
 \label{eq:scenario_cost}
\end{align}
The finite-scenario robust quadratic program is
\begin{align}
 \min_{\Delta\vect\Theta_j}\quad&
 \sum_{s=1}^{N_p}\omega_s J_j^{(s)}
 \label{eq:slow_qp}\\
 \mathrm{s.t.}\quad&
 \text{\eqref{eq:closed_loop_lifted}, \eqref{eq:orientation_recursion}},
 \quad s=1,\ldots,N_p,
 \nonumber\\
 &F_{\min}+\sigma_F^{(s)}
 \leq
 \widehat F_{n,j+r,q|j}^{(s)},
 \nonumber\\
 &\widehat F_{n,j+r,q|j}^{(s)}
 \leq
 F_{\max}-\sigma_F^{(s)},
 \nonumber\\
 &q=1,\ldots,m,\quad
 r=0,\ldots,N-1,
 \nonumber\\
 &s=1,\ldots,N_p,
 \nonumber\\
 &\vect\theta_0+\vect\vartheta_{j+r|j}\in\Theta,
 \nonumber\\
 &\Delta\vect\theta_{j+r|j}\in\Delta\Theta,
 \quad r=0,\ldots,N-1.
 \nonumber
\end{align}
Here $\widehat F_{n,j+r,q|j}^{(s)}$ denotes the $q$th component of the stacked fast-rate force prediction \eqref{eq:closed_loop_force_stack}, and $\sigma_F^{(s)}>0$ bounds the additive force-prediction error not represented by scenario $p^{(s)}$. The weights satisfy $W_I\succeq0$, $w_F\geq0$, $R\succ0$, and $\omega_s\geq0$ with $\sum_s\omega_s=1$. Because the model bank is finite, the predictions are affine, the constraints are linear, and the objective is quadratic, \eqref{eq:slow_qp} is a convex QP.

Image error is treated as a performance objective rather than a hard safety variable, so no artificial image-quality slack variable is needed. Only the first orientation increment is applied,
\begin{equation}
 \vect\vartheta_j
 =
 \vect\vartheta_{j-1}
 +\Delta\vect\theta_{j|j}^{\star},
\end{equation}
and the resulting orientation is held during the next image interval. If the QP is infeasible, no unconstrained tilt step is issued; the last admissible orientation is held while the fast safety layer remains active, and persistent infeasibility triggers the supervisor.

If the image available at slow update $j$ has age $d_j>\bar d_I$ or fails the validity test, the slow optimization is not updated from that image. Baseline B2 uses the same image feature and orientation-rate limits but applies the static update
\begin{equation}
 \Delta\vect\theta_j
 =
 -K_I\vect e_I(\ell_j),
 \label{eq:baseline_image}
\end{equation}
without timestamp-based state reconstruction, explicit force prediction, or delay/coupling compensation.

\subsection{Sample-Wise Force Safety Filter}

The slow QP limits predicted force over each fast sample in its horizon, but a separate fast safety layer has priority over the performance controller. Define the scalar barrier functions
\begin{equation}
 h_1(F)=F-F_{\min},
 \qquad
 h_2(F)=F_{\max}-F,
 \label{eq:barrier_functions}
\end{equation}
and let $h_i(k):=h_i(F_n(k))$. At each fast update, the applied command is obtained from
\begin{align}
 u_{n,k}
 =
 \arg\min_{u\in\mathcal U_n}\quad&
 \left(u-u_{n,k}^{0}\right)^2
 \label{eq:safety_projection}\\
 \mathrm{s.t.}\quad&
 h_i\!\left(F_{n,k+1}^{(s)}(u,w)\right)
 \geq
 (1-\alpha_i)h_i(k),
 \nonumber\\
 &i\in\{1,2\},
 \quad
 s=1,\ldots,N_p,
 \quad
 \forall w\in\mathcal W_F,
 \nonumber
\end{align}
where $0<\alpha_i\leq1$, $\mathcal U_n$ is the actuator-admissible interval, and $\mathcal W_F$ is the bounded additive one-step force-prediction error. For the scalar affine force model and interval-bounded $w$, the worst-case forms of the constraints in \eqref{eq:safety_projection} are linear inequalities in $u$, so the safety projection is a one-dimensional convex QP.

If \eqref{eq:safety_projection} is infeasible, the force limits are not relaxed. Instead, normal operation is terminated and the independent supervisor commands a predefined controlled retraction.

\subsection{Conditional Boundedness and Force-Constraint Preservation}

The following result states local sufficient conditions to be checked using the identified model bank and validation residuals. It is a control-theoretic statement within the operating assumptions of Section~\ref{sec:system}, not an unconditional clinical-safety guarantee.

\noindent\textbf{Proposition 1.}
Suppose A1--A5 hold and the true local dynamics are represented by the accepted model bank plus the stated additive residual bounds. For each $p^{(s)}\in\mathcal P$, define the unsaturated PI force-loop matrix
\begin{equation}
 A_F^{(s)}
 =
 \begin{bmatrix}
 a^{(s)}-b^{(s)}K_p & -b^{(s)}K_i\\
 T_f & 1
 \end{bmatrix}.
 \label{eq:fast_closed_loop_matrix}
\end{equation}
Assume there exist matrices $P_F=P_F^{\mathsf T}\succ0$ and $Q_F=Q_F^{\mathsf T}\succ0$ such that
\begin{equation}
 A_F^{(s)\mathsf T}P_FA_F^{(s)}-P_F
 \preceq
 -Q_F,
 \qquad
 s=1,\ldots,N_p.
 \label{eq:common_lyapunov_condition}
\end{equation}
Then the nominal PI force loop is uniformly exponentially stable over the model bank, and bounded residual coupling, disturbance-estimation error, and model mismatch produce a bounded force-loop state.

At the slow sampling instants, let $\vect z_F(j)$ denote the lifted force-loop state and let $\vect e_I(j)$ denote the image-error state. Suppose that, for every feasible slow update in the certified local region, the receding-horizon law and the lifted force subsystem admit finite-gain bounds of the form
\begin{align}
 \norm{\vect z_F}_{\infty,[0,J]}
 \leq{}&
 c_F\norm{\vect z_F(0)}
 +\gamma_{FI}\norm{\vect e_I}_{\infty,[0,J]}
 +\gamma_{Fw}\bar w,
 \label{eq:force_gain_bound}\\
 \norm{\vect e_I}_{\infty,[0,J]}
 \leq{}&
 c_I\norm{\vect e_I(0)}
 +\gamma_{IF}\norm{\vect z_F}_{\infty,[0,J]}
 +\gamma_{Iv}\bar v,
 \label{eq:image_gain_bound}
\end{align}
for all finite horizons $J$, where $\bar w$ and $\bar v$ bound the accepted force-side and image-side residuals. If
\begin{equation}
 \gamma_{FI}\gamma_{IF}<1,
 \label{eq:small_gain_condition}
\end{equation}
then the interconnected force--image error dynamics are locally finite-gain stable. Define
\begin{align}
 \eta_F={}&
 c_F\norm{\vect z_F(0)}
 +\gamma_{FI}c_I\norm{\vect e_I(0)}
 \nonumber\\
 &+\gamma_{Fw}\bar w
 +\gamma_{FI}\gamma_{Iv}\bar v.
 \label{eq:force_bound_numerator}
\end{align}
Then
\begin{equation}
 \norm{\vect z_F}_{\infty,[0,J]}
 \leq
 \frac{\eta_F}{1-\gamma_{FI}\gamma_{IF}}.
 \label{eq:explicit_force_bound}
\end{equation}
A corresponding bound for $\vect e_I$ follows by substitution into \eqref{eq:image_gain_bound}.

Finally, if $F_n(0)\in[F_{\min},F_{\max}]$, the true one-step force evolution is covered by the model bank plus $\mathcal W_F$, and the safety projection \eqref{eq:safety_projection} remains feasible, then the interval $[F_{\min},F_{\max}]$ is positively invariant.

\noindent\textit{Proof sketch.}
Condition \eqref{eq:common_lyapunov_condition} provides a common quadratic Lyapunov function $V_F=\vect\zeta_F^{\mathsf T}P_F\vect\zeta_F$ for $\vect\zeta_F=[e_F\;\xi]^{\mathsf T}$ over the finite model bank. The residual orientation-coupling error, disturbance-estimation error in \eqref{eq:disturbance_error_bound}, and additive model mismatch enter as bounded inputs, yielding the first finite-gain inequality after lifting to the slow timescale. The feasible slow receding-horizon law and local image model yield the second finite-gain inequality on the certified trust region. Combining \eqref{eq:force_gain_bound} and \eqref{eq:image_gain_bound} gives \eqref{eq:explicit_force_bound} whenever \eqref{eq:small_gain_condition} holds. For constraint preservation, \eqref{eq:safety_projection} gives
\begin{equation}
 h_i(k+1)\geq(1-\alpha_i)h_i(k)\geq0,
\end{equation}
for both barrier functions whenever the robust safety problem is feasible. Induction therefore gives $F_n(k)\in[F_{\min},F_{\max}]$ for all subsequent samples.

The proposition does not establish recursive feasibility of the slow QP because no terminal invariant set or equivalent recursive-feasibility mechanism is imposed in \eqref{eq:slow_qp}. Slow-QP infeasibility, persistent safety-filter intervention, contact loss, excessive tangential moment, image-feature degeneracy, stale images, wrench-sensor faults, or departure from the identified trust region are handled by the supervisor.

\begin{figure}[t]
    \centering
    \fbox{\parbox[c][1.06in][c]{0.94\columnwidth}{\centering
    \tbd{Fig. 3: fast force loop, timestamped image reconstruction, closed-loop lifted predictor, finite-scenario QP, sample-wise safety projection, and supervisory override.}}}
    \caption{Dual-rate control architecture. The final diagram will identify the fast and slow sample rates, image age, held orientation command, closed-loop lifted predictor, safety-filter path, and image-independent supervisory override.}
    \label{fig:controller_placeholder}
\end{figure}

The supervisor independently monitors normal force, tangential moment, contact loss, image age and validity, wrench-sensor health, joint and workspace margins, communication state, and controller watchdog timing. Fault thresholds, retraction velocity, state-reset logic, and re-entry conditions are fixed before comparative controller experiments.


==> sections_v1/05_validation_results.tex <==
% Final compact ACC-ready revision of Section V.
% Assumes \result{.}, \tbd{.}, \vect{.}, \norm{.}, booktabs, and graphicx.

\section{Experimental Validation}
\label{sec:validation}

\subsection{Protocol and Metrics}
Validation tested four questions: whether the identified model predicts held-out force--orientation--image transients; whether coupling/delay compensation improves force regulation; whether image feedback improves the controlled view feature without degrading the force constraint; and whether safety interventions agree with the declared local operating envelope. Three controllers were compared: force-only control (B1), the static image update in \eqref{eq:baseline_image} (B2), and the proposed dual-rate controller (P). All used the same force reference, actuator limits, force-safety layer, and supervisor; B2 and P used the same image feature and orientation-rate limits. Hence P--B2 isolates the multirate predictor, while B2--B1 isolates image feedback.

The primary study used two tissue-mimicking contact conditions under \tbd{static, repeatable vertical-motion, and combined motion/tilt conditions}. Each controller--condition cell contained \tbd{$N_{\rm tr}$} complete trials across \tbd{$N_b$} independently re-established contact blocks, with controller order randomized within blocks. Disturbance motion was independently measured, and all gains, model-bank scenarios, residual bounds, image-validity thresholds, and safety limits were frozen before comparison. A preliminary volunteer-tissue study was also performed under University of Alabama IRB Protocol 24-01-7231; those data are secondary, are not used for tuning, and are reported descriptively.

The primary endpoint was trial-level force RMSE during dynamic motion. Secondary outcomes were RMS image-feature error, peak force, time outside the nominal force band, recovery time, safety-filter/QP activity, supervisor stops, and computation time. Complete trials were the independent units; frame-level samples were not treated as replicates. Paired controller differences are reported with $95\%$ confidence intervals, with block/site effects modeled only when the number of independent blocks supports such inference.

\subsection{Results}
Table~\ref{tab:validation_summary} consolidates the model/certificate checks required by Proposition~1 and the primary controller outcomes. On held-out trials, the model achieved \result{force prediction error} and \result{image prediction error}, with accepted force residual bound \result{$\sigma_F$}, admissible image age \result{$\bar d_I$}, and orientation sensitivity \result{$\sigma_{\min}(L_\theta)$}. The common Lyapunov test was \result{status/margin}, and the evaluated local gain product was \result{$\gamma_{FI}\gamma_{IF}$}; the boundedness claim is invoked only over the corresponding validated region.

In the primary dynamic condition, P changed force RMSE by \result{P--B2 effect with 95\% CI} relative to B2 and image-feature RMS by \result{P--B2 effect with 95\% CI}, while peak force and out-of-band time were \result{results}. Figure~\ref{fig:validation_results} shows a representative synchronized trial and trial-level comparisons across disturbances. Removing \result{coupling compensation / timestamp reconstruction / tightening / disturbance estimation} caused the largest deterioration in \result{metric}. The safety filter intervened in \result{count/fraction} of trials, the slow QP was infeasible in \result{count/fraction}, and \result{count} supervisor retractions occurred; interventions were \result{relation to predicted boundary}. Median QP time was \result{value} ms, below the \result{value}-ms image-update interval. Volunteer trials ($n=\result{value}$) showed \result{brief feasibility result} and were not pooled with the phantom analysis.

\begin{table}[t]
\caption{Compact validation summary. Trial-level statistics use complete trials/blocks, not frames.}
\label{tab:validation_summary}
\centering
\footnotesize
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{lccc}
\toprule
Quantity & B1 & B2 & P \\
\midrule
\multicolumn{4}{l}{\emph{Model/certificate checks}}\\[-1mm]
Force prediction error & -- & -- & \result{--} \\
Image prediction error & -- & -- & \result{--} \\
$\sigma_F$, $\bar d_I$ & -- & -- & \result{--} \\
$\sigma_{\min}(L_\theta)$ & -- & -- & \result{--} \\
Lyapunov / $\gamma_{FI}\gamma_{IF}$ & -- & -- & \result{--} \\
\midrule
\multicolumn{4}{l}{\emph{Primary dynamic condition}}\\[-1mm]
Force RMSE (N) & \result{--} & \result{--} & \result{--} \\
Image RMS (\tbd{unit}) & \result{--} & \result{--} & \result{--} \\
Peak force (N) & \result{--} & \result{--} & \result{--} \\
Out-of-band time (\%) & \result{--} & \result{--} & \result{--} \\
Supervisor stops & \result{--} & \result{--} & \result{--} \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[t]
    \centering
    \IfFileExists{fig_validation_results.pdf}{%
    \includegraphics[width=0.99\columnwidth]{fig_validation_results.pdf}%
    }{%
    \fbox{\parbox[c][1.68in][c]{0.94\columnwidth}{\centering
    \textbf{Fig. 4 placeholder:} (a) synchronized raw force and limits for B1/B2/P; (b) image-feature error and tilt for B2/P; (c) trial-level force/image performance and ablation/safety summary across disturbances.}}}
    \caption{Dynamic hardware validation. Metrics are computed from raw synchronized logs; filtered traces, if shown, are visualization only. The identified trust region is distinguished from extrapolation.}
    \label{fig:validation_results}
\end{figure}


==> sections_v1/06_discussion.tex <==
% Final compact ACC-ready revision of Section VI.

\section{Discussion}
\label{sec:discussion}

The contribution should be interpreted as explicit control of \emph{multirate coupling}, not as the first combination of image and force feedback. Image servoing, force/orientation regulation, and image-dependent force adaptation are already established in robotic ultrasound \cite{jiang2020normal,jiang2021force,akbari2021,zakeri2025,piedra2026}. Here, P--B2 quantifies the value of predicting the force consequence of an orientation update before the corresponding image becomes available, whereas B2--B1 quantifies the value of image feedback itself. The ablations are therefore essential: lower force RMSE without preserved image performance would indicate aggressive compliance rather than coordinated imaging, while lower image error with higher peak force would expose an unfavorable trade-off.

The theory is intentionally local. Proposition~1 is invoked only for the model bank, residual bounds, image-age limit, and image-sensitivity region summarized in Table~\ref{tab:validation_summary}. Repeated safety intervention well inside that region would indicate underestimated uncertainty; infeasible slow QPs are reported rather than resolved by relaxing force limits. The independent force-safety/supervisory path is therefore part of the contribution, because image failure cannot directly disable contact protection.

The main limitations are the local linearization, the use of an image-feature surrogate rather than diagnostic quality, and the gap between repeatable phantoms and living tissue. Slip, hysteresis, large rotations, abrupt geometry, or loss of acoustic visibility can invalidate the identified model. The volunteer study is accordingly feasibility evidence only. Broader translation requires subject-level validation across anatomies and scanners, clinician-defined force/image endpoints, and re-identification of uncertainty and timing bounds.


==> sections_v1/07_conclusion.tex <==
% Final compact ACC-ready revision of Section VII.

\section{Conclusion}
\label{sec:conclusion}
This paper formulated robotic ultrasound interaction as a delayed multirate force--image control problem and combined an identified closed-loop predictor with fast force regulation, constrained image-guided orientation updates, and image-independent contact protection. Within the validated local region, the analysis gives conditional practical boundedness and force-constraint invariance; experiments show \result{primary force result} while \result{image/safety result}. Claims are restricted to the tested force, motion, orientation, tissue, and latency ranges; future work will extend the model and evaluate subject- and task-level clinical generalization.

\section*{Acknowledgment}
The authors gratefully acknowledge support from the University of Alabama faculty startup fund and the Alabama Transportation Institute. This work was also supported by the U.S. Department of Transportation, Office of the Assistant Secretary for Research and Technology, University Transportation Centers Program, through the Center for Regional and Rural Connected Communities (CR2C2), Grant No.~69A3552348304.

==> sections_v2/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Brightness mode (B-mode) ultrasound provides real-time, radiation-free imaging with comparatively low cost, but its image quality is strongly coupled to how the probe interacts with the tissue. During manual scanning, a sonographer continuously
coordinates probe position and orientation with contact force while responding to local surface geometry, tissue compliance, and the observed ultrasound image. Robotic ultrasound, therefore, presents a coupled sensing-and-control problem rather than a conventional trajectory-following task. Existing reviews accordingly identify scanning-path generation, probe-tissue force regulation, and image-quality or orientation optimization as central components of autonomous robotic ultrasound systems \cite{li2021overview,haxthausen2021,salcudean2022,jiang2023review}. More recent surveys note two remaining limitations that are particularly relevant from a control perspective: interaction wrench components associated with probe orientation are often simplified, and real-time ultrasound feedback remains less commonly integrated into online scan optimization \cite{bi2024,munir2025,han2025clinical}. 
% These limitations motivate control architectures in which the probe-tissue dynamics, cross-coupling between controlled variables, and heterogeneous sensing rates are treated explicitly. 

Early image-guided robotic ultrasound demonstrated that features extracted directly from ultrasound images can close the robot-positioning loop \cite{abolmaesumi2002}. Subsequent visual-servoing approaches optimized ultrasound confidence measures to improve acoustic coupling and probe orientation \cite{chatelain2015}. In parallel, interaction-force information has been exploited for estimating the local surface normal and regulating probe orientation \cite{jiang2020normal,jiang2021force,ma2022asee}. More recent explicit force-control strategies directly regulate contact forces and moments to achieve responsive probe - tissue interaction under heterogeneous and dynamic conditions \cite{piedra2026}. Ultrasound feedback has also enabled autonomous entering and alignment of tubular structures \cite{jiang2022tubular}, while image-quality estimated have been used to adapt the commanded contact force rather than maintaining a fixed force across different imaging conditions \cite{akbari2021,zakeri2025}. Collectively, these studies establish that image and force sensing provide complementary information. Consequently, simply combining the two feedback modalities is no longer, by itself, sufficient to contribute to control. 

Learning-based approaches have further expanded the achievable level of autonomy. Deep reinforcement learning has been used to navigate toward anatomical targets from ultrasound observations \cite{hase2020}; reinforcement learning policies have combined visual scene perception with compliant force control for scanning moving, markerless targets \cite{ning2021rl}; and inverse reinforcement learning has transferred active-compliance behavior to uncertain soft environments \cite{ning2024irl}. Constraint-aware policy optimization explicitly incorporates interaction-force limits during policy learning \cite{duan2025safe}, while recent large-scale imitation learning has demonstrated substantial generalization across an autonomous carotid-ultrasound workflow \cite{jiang2025ultrabot}. These developments demonstrate the potential of learning for perception, decision making, and reference generation. At the same time, recent reviews emphasize limitations associated with medical-data availability, domain variation, and insufficient incorporation of physical knowledge \cite{bi2024,yip2023}. For contact-rich medical robotics, this suggests a useful separation of roles: learned perception can provide task-relevant image information, whereas the high-bandwidth interaction loop should retain sufficient physical structure to support constraint enforcement, robustness analysis, and failure detection. 

A control issue that is less explicitly addressed in this literature is the multirate dynamic coupling between force regulation and image-guided probe correction. Robot state and wrench measurements can be updated at high rates, whereas B-mode images are acquired, transferred, and processed at substantially lower rates and with non-negligible latency. This mismatch has already appeared in practical robotic ultrasound implementations; for example, image-based force adjustment has been implemented with a slower image-quality loop than the underlying robot-control loop \cite{akbari2021}. The difficulty is more fundamental than asynchronous sensing alone. An orientation correction computed from an image changes probe indentation, the contact moment, and consequently the normal force before a new image measurement becomes available. Conversely, a fast force regulator reacts to the normal displacement induced by the orientation update and can partially oppose the intended image-based correction. Tissue stiffness, local curvature, surface motion, and uncertainty in image sensitivity further modify this bidirectional interaction. Recent dual-loop approaches have demonstrated image-dependent force adaptation and robust contact-force tracking \cite{zakeri2025}, while explicit force/moment regulation improves dynamic interaction performance \cite{piedra2026}. In addition, Li et al. \cite{li2026trajectory} explicitly incorporate trajectory-dependent feedforward and delay compensation for dynamic contact-force tracking, and Qian et al. \cite{qian2026symmetry} combine image guidance with biomechanics-informed force estimation/control. However, these advances do not directly formulate the image-guided orientation loop and the high-rate force loop as an identified, delayed multirate system whose cross-coupling can be predicted and incorporated into controller design. 


This paper addresses this control gap through a model-informed dual-rate framework for dynamic robotic ultrasound interaction. Rather than pursuing end-to-end autonomous diagnosis, we focus on a narrower control objective: coordinating normal interaction force with an ultrasound-derived orientation feature while explicitly accounting for probe-tissue coupling, image latency, model uncertainty, and operational constraints. A local input-output model is identified from bounded excitation experiments and lifted to the image-update timescale, allowing the slower image-guided controller to predict the force consequences of orientation corrections while a faster inner loop regulates probe-tissue contact. This structure preserves high-rate interaction control while using ultrasound information where it is most informative. The main contributions are:

\vspace{-0.5 mm}
\begin{enumerate}
    \item a locally identified and independently validated force--pose--image model that captures normal compliance, orientation-to-force coupling, image sensitivity, transport delay, and bounded uncertainty, together with a lifted representation that preserves within-interval force predictions;
    
    \item a dual-rate controller that combines high-rate disturbance-compensated force regulation with delayed, constraint-aware image updates, plus sufficient local boundedness and feasibility conditions, and an image-independent contact supervisor; and
    
    \item repeated hardware comparisons with force-only and decoupled force--image baselines under dynamic phantom contact, supported by ablations of coupling compensation and delay handling and by separate volunteer-tissue feasibility tests.
\end{enumerate}

%The resulting framework is intended to bridge high-bandwidth interaction control and lower-rate image-guided adaptation without requiring either loop to be collapsed into a single-rate controller or an end-to-end learned policy.


==> sections_v2/02_system_problem.tex <==
\section{System and Problem Formulation}
\label{sec:system}

\subsection{Physical Platform, Contact Variables, and Timing}
The platform combines a Kinova manipulator, a rigidly mounted ultrasound probe, six-axis force/torque sensing, and B-mode imaging. Robot/wrench signals are sampled at $f_f=1000$ Hz and images at $f_I=25$ Hz; acquisition-to-processing latency is $\tau_I=20$--$30$ ms with bounded jitter. All streams share a common clock. 

Let $q\in\mathbb R^{n_q}$ denote the robot joint coordinates and let $J_P(q)$ denote the Jacobian associated with the probe reference frame. The rigid-body manipulator dynamics are written in the standard form
\begin{equation}
M(q)\ddot {q}+C(q,\dot {q})\dot {q}+g(q)
=\tau+J_P^\top(q)\,{}^{B}\!h_c ,
\label{eq:robot_dyn}
\end{equation}
where $\tau$ is the commanded joint torque and ${}^{B}\!h_c=[{}^{B}\! F_c^\top,\;{}^{B}\!\mu_c^\top]^\top$ is the external contact wrench exerted by the environment on the robot, expressed about the probe reference point in the robot-base frame $\{B\}$. The low-level robot servo is not redesigned in this study; instead, it provides a stable operational-space interface for probe-normal translation and probe orientation, following the operational-space separation of motion and interaction forces introduced by Khatib \cite{khatib1987}.

Let $\{B\}$, $\{S\}$, and $\{P\}$ denote the robot-base, wrench-sensor, and probe frames. The measured sensor wrench is first transformed to $\{P\}$, compensated for probe payload and sensor bias, and then expressed in $\{B\}$:
\begin{equation}
{}^{B}\!h_c
={}^{B}\!X_P^{*}
\left(
{}^{P}\!X_S^{*}\,{}^{S}\!h_m
-{}^{P}\!h_g(q)-{}^{P}\!b_h
\right),
\label{eq:wrench_comp}
\end{equation}
where $X^{*}$ denotes the dual-adjoint wrench transformation, ${}^{P}\!h_g(q)$ is the orientation-dependent payload/gravity wrench of the probe assembly, and ${}^{P}\!b_h$ is the calibrated sensor bias. Recomputing the gravity term during probe rotation prevents payload effects from being interpreted as probe--tissue coupling.

\subsection{Local Contact Geometry and Multirate Measurements}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.94\columnwidth]{demo_force_tracking.jpg}
    \caption{Robotic-ultrasound platform, representative B-mode image, and demonstration force trace. Quantitative comparisons use the randomized validation protocol in Section~\ref{sec:validation}.}
    \label{fig:system}
\end{figure}

Let $e_n=[0\;0\;1]^\top$ denote the probe-normal axis in $\{P\}$, chosen to point from the probe face into tissue. Its base-frame representation is
\begin{equation}
{}^{B}\!n(\theta)={}^{B}\!R_P(\theta)e_n ,
\label{eq:normal}
\end{equation}
where $\theta\in\mathbb R^{n_\theta}$ contains the measured one or two controlled tilt angles. For probe-face point ${}^{B}\!p_e$ and the corresponding local undeformed surface point ${}^{B}\!p_s$, define
\begin{equation}
\delta={}^{B}\!n^\top(\theta)
({}^{B}\!p_e-{}^{B}\!p_s),\qquad
F_n=-{}^{B}\!n^\top(\theta)\,{}^{B}\!F_c .
\label{eq:contact}
\end{equation}
Thus $\delta>0$ and $F_n>0$ denote compression. The tangential contact moment,
\begin{equation}
\mu_t=
\left(I-{}^{B}\!n\,{}^{B}\!n^\top\right){}^{B}\!\mu_c ,
\label{eq:tangent_moment}
\end{equation}
is monitored by the independent supervisor. The moment is evaluated on the same probe reference point used in \eqref{eq:robot_dyn}--\eqref{eq:wrench_comp}. Force- and moment-based cues have previously been used to estimate local probe alignment and regulate contact in robotic ultrasound \cite{jiang2020normal, jiang2021force, piedra2026}.

The fast force loop executes at $t_k=kT_f$, with $T_f=f_f^{-1}$. The nominal image period is
\begin{equation}
T_I=mT_f,\qquad m\in\mathbb N.
\label{eq:rates}
\end{equation}
The $j$th image is captured at $t_j^c=jT_I+\epsilon_j^c$ and becomes available at $t_j^a=t_j^c+\tau_j$, where $\epsilon_j^c$ is bounded acquisition jitter and $\tau_j$ is acquisition-to-processing latency. At slow update $t_j^s=jT_I$, the newest valid image available to the controller has index
\begin{equation}
\ell_j=\max\{\ell:t_\ell^a\le t_j^s\},\qquad
d_{I,j}=j-\ell_j .
\label{eq:image_age}
\end{equation}
Nominal image-guided operation requires $0\le d_{I,j}\le\bar d_I$; larger image age, repeated frame loss, or invalid image quality invokes supervisory logic. The need to coordinate a slower image-dependent adaptation layer with a faster contact-force regulation has also appeared in prior robotic-ultrasound systems \cite{akbari2021, zakeri2025}; recent dynamic force-control work further highlights the importance of explicit delay compensation during robotic ultrasound contact \cite{li2026trajectory}.

Let $s_I(I_j)\in\mathbb R^{n_I}$ be an orientation-sensitive image feature associated with the image capture time. Define
\begin{equation}
e_F(k)=F_n(k)-F_d,\qquad
e_I(j)=s_I(I_j)-s_{I,d},
\label{eq:errors}
\end{equation}
where the force reference $F_d$ is constant in the present experiments. For time-varying force references, the known reference increment is included explicitly in the prediction model. Let
\begin{equation}
\vartheta_j=\theta_{d,j}-\theta_0,\qquad
\Delta\theta_j=\vartheta_j-\vartheta_{j-1},
\label{eq:orientation}
\end{equation}
where $\theta_0$ is the nominal probe orientation. Thus $\vartheta_j$ is held during image interval $j$, whereas $\Delta\theta_j$ is the image-rate orientation update. Then, the controller enforces
\begin{equation}
F_{\min}\le F_n\le F_{\max},\qquad
\theta_d\in\Theta,\qquad
\Delta\theta\in\Delta\Theta .
\label{eq:hard_limits}
\end{equation}
The moment limit $\|\mu_t\|\le\mu_{\max}$ is monitored by the supervisor rather than predicted by the slow optimization.

\subsection{Local Operating Assumptions and Control Objective}

The proposed controller is intentionally local. Its operating region is defined by the following assumptions. \textbf{A1:} Probe--tissue contact is maintained on a continuously differentiable local surface patch. \textbf{A2:} Local stiffness, damping, surface velocity, model residuals, and sensing errors are bounded over the validated operating region. \textbf{A3:} Image jitter and processing latency are bounded and $d_{I,j}\le\bar d_I$ during nominal image-guided operation. \textbf{A4:} The selected image feature is locally Lipschitz in force and orientation. For the active controlled axes, $n_I\ge n_\theta$ and the identified orientation sensitivity satisfies
$\sigma_{\min}(L_\theta)\ge\underline\sigma_\theta>0$. \textbf{A5:} The underlying robot motion interface is internally stable over the commanded range, and every accepted local force model has a known positive control direction $b^{(s)}\ge b_{\min}>0$.

The objective is to regulate normal force at a fast rate while reducing the image-feature error through slower orientation updates. Force, orientation, and orientation-rate limits are explicitly constrained. Contact loss, excessive tangential moment, stale or invalid images, image-feature degeneracy, workspace violations, sensor faults, communication faults, or departure from the validated local region are supervisory events rather than nominal convergence cases.


==> sections_v2/03_model_identification.tex <==
\section{Local Modeling and System Identification}

\subsection{Local Force--Pose Model}

Within a bounded contact patch, probe--tissue interaction is locally motivated by a Kelvin--Voigt relation and a first-order geometric approximation. This intentionally low-order representation is consistent with the broader use of physically structured local contact models in force regulation, where the objective is control-relevant prediction rather than a global constitutive description of tissue \cite{zakeri2025, piedra2026}. 
\begin{equation}
F_n\approx k(\rho)\delta+c(\rho)\dot\delta+F_0,\qquad
\delta\approx\delta_0+\Delta p_n+r_\theta^\top\vartheta+d_s ,
\label{eq:kv}
\end{equation}
where $k(\rho)>0$ and $c(\rho)\ge0$ are local effective stiffness and damping, $F_0$ is the nominal preload, $r_\theta$ maps small probe rotations to effective indentation, and $d_s$ is signed local surface displacement, positive when it increases indentation. Equation~\eqref{eq:kv} motivates the model structure but is not treated as a global biomechanical tissue law.

For control and prediction, each accepted local condition is represented directly by a low-order, scenario-indexed deviation model
\begin{equation}
e_F(k+1)
=a^{(s)}e_F(k)+b^{(s)}u_{n,k}
+g^{(s)\top}\vartheta_{j(k)}
+d_{F,k}+r^{(s)}_{F,k},
\label{eq:force_model}
\end{equation}
where $j(k)=\lfloor k/m\rfloor$, $u_{n,k}$ is the incremental normal command, $d_{F,k}$ is a slowly varying lumped disturbance, and $r^{(s)}_{F,k}$ is the remaining prediction error. The model coefficients are treated as fixed over a prediction interval for each scenario $s$; changes in local contact condition are represented by switching among the finite accepted model banks rather than by using a time-varying matrix power inside one lifted interval. The sign convention in A5 gives $b^{(s)}>0$.

\subsection{Image Feature Dynamics}

For probe-normal alignment, an acoustic-confidence map $Q(I_j)$ is divided into opposing regions. Ultrasound confidence maps were introduced as per-pixel measures of signal reliability under attenuation and shadowing \cite{karamalis2012ultrasound}, and were subsequently used for ultrasound visual servoing and automatic
probe-normal positioning \cite{chatelain2015, jiang2020normal}. A representative two-axis feature is
\begin{equation}
s_I(I_j)=
\begin{bmatrix}
\bar Q_L-\bar Q_R\\
\bar Q_U-\bar Q_D
\end{bmatrix},
\label{eq:image_feature}
\end{equation}
where $\bar Q_\bullet$ denotes the mean normalized confidence in the corresponding fixed image region. If only one tilt axis is observable, only the associated feature component is retained. Global image metrics such as mean confidence, contrast-to-noise ratio, or entropy are treated as evaluation quantities unless they are explicitly included in the controlled feature.

Around the nominal operating point $(\theta_0,F_d,s_{I,d})$, the slow image dynamics for scenario $s$ are identified as
\begin{equation}
e_I(j+1)
=A_I^{(s)}e_I(j)
+L_\theta^{(s)}\Delta\theta_j
+L_F^{(s)}\bar e_F(j)
+r^{(s)}_{I,j},
\label{eq:image_model}
\end{equation}
with
\begin{equation}
\bar e_F(j)=\frac{1}{m}\sum_{q=0}^{m-1}e_F(jm+q).
\label{eq:mean_force}
\end{equation}
Because \eqref{eq:image_model} is a deviation model, using force error rather than absolute force is consistent with identification around the fixed nominal force $F_d$. The residual $r^{(s)}_{I,j}$ includes local linearization and unmodeled image-response error; image measurement noise is treated separately below.

\subsection{Timestamped Image Reconstruction}

At slow update $j$, the newest available image is generally not the current nominal frame. Denote its measured feature error by
\begin{equation}
y_{I,\ell_j}=e_I(\ell_j)+\nu_{I,\ell_j},
\label{eq:image_meas}
\end{equation}
where $\nu_I$ is image-feature measurement noise. Since all orientation updates and force summaries after frame $\ell_j$ are known, the image state is propagated forward recursively:
\begin{align}
\hat e_{I,\ell_j|j}&=y_{I,\ell_j},\nonumber\\
\hat e_{I,r+1|j}
&=\hat A_I\hat e_{I,r|j}
+\hat L_\theta\Delta\theta_r
+\hat L_F\bar e_F(r),
\, r=\ell_j,\ldots,j-1.
\label{eq:image_recon}
\end{align}
For $d_{I,j}=0$, \eqref{eq:image_recon} reduces to the current image measurement. Reconstruction uncertainty increases with image age; its accepted bound is obtained from held-out data for $0\le d_{I,j}\le\bar d_I$. If that delay range or the image-validity test is violated, the image-guided update is withheld. This explicit timestamp treatment is motivated by the practical separation between image acquisition/processing and robot-force update rates in robotic ultrasound \cite{akbari2021, li2026trajectory}. 

\subsection{Identification, Model Bank, and Residual Bounds}

Bounded normal and tilt excitations are applied around a nominal phantom contact condition, followed by combined excitation to expose force--orientation coupling. Excitation amplitudes and spectra are selected to cover the intended control bandwidth while respecting predetermined force, moment, pose, and velocity limits. Image latency is measured independently so that transport delay is not absorbed into the fitted dynamic coefficients.

Force and image parameters are estimated separately by regularized least squares. Using $q\in\{F,I\}$ to denote the subsystem,
\begin{equation}
\hat\Theta_q
=
\arg\min_{\Theta_q}
\sum_{r\in\mathcal T_q}
\|y_{q,r+1}-\Theta_q\phi_{q,r}\|_{W_q}^2
+\lambda_q\|\Theta_q\|_F^2 .
\label{eq:ridge}
\end{equation}
Representative regressors are
\[
\phi_{F,k}
=\mathrm{col}\!\left(e_F(k),u_{n,k},\vartheta_{j(k)}\right),\,\,
\phi_{I,j}
=\mathrm{col}\!\left(e_I(j),\Delta\theta_j,\bar e_F(j)\right).
\]
Training and validation are separated by complete trials and re-established contact locations, not by adjacent samples. Candidate models are evaluated using held-out multi-step prediction error, residual bias/autocorrelation, numerical conditioning, and parameter variation across contact sites. This emphasis on
independent validation and control-relevant model complexity
follows standard system-identification principles \cite{ljung2010perspectives}.

Accepted fits form the finite model bank
\begin{equation}
\mathcal P=\{p^{(1)},\ldots,p^{(N_p)}\}.
\label{eq:model_bank}
\end{equation}
For each scenario, held-out force-prediction errors are summarized by horizon-dependent bounds $\varepsilon_{F,h}^{(s)}$ for prediction step $h$. The one-step value $\varepsilon_{F,1}^{(s)}$ is used by the fast safety filter, whereas the slow optimizer uses the bound corresponding to each predicted fast sample. Image-side prediction/reconstruction error is likewise bounded over the accepted image-age range. The manuscript should state the exact construction rule used in experiments, e.g., a maximum held-out absolute error plus a pre-specified margin or an independently calibrated high-confidence bound. These quantities define a \emph{validated local operating region}, not a global certificate for arbitrary anatomy.

\begin{figure}[t]
\centering
\fbox{\parbox[c][0.82in][c]{0.94\columnwidth}{\centering
\textbf{Identification/validation figure placeholder}\\
bounded excitation $\rightarrow$ trial-level train/validation split $\rightarrow$ held-out force/image prediction $\rightarrow$ residual bounds and accepted model bank}}
\caption{Identification and held-out validation used to define the finite local model bank and prediction-error bounds.}
\label{fig:id}
\end{figure}

==> sections_v2/04_control.tex <==
\section{Dual-Rate Constrained Control}

\subsection{Fast Normal-Force Regulation}

The existing normal-force controller without image-informed coupling compensation is retained as baseline B1. High-bandwidth force regulation, probe alignment, and explicit force/moment control are established components of
robotic-ultrasound interaction control \cite{jiang2021force, zakeri2025, piedra2026}. The proposed nominal fast controller is
\begin{equation}
u^0_{n,k}
=
-K_p e_F(k)-K_i\xi_k
-\hat b^{-1}\hat g^\top\vartheta_{j(k)}
-\hat b^{-1}\hat d_{F,k},
\label{eq:fast_control}
\end{equation}
where $K_p,K_i>0$, $\xi_k$ is the integral state, and $\hat b,\hat g$ are nominal identified coefficients. No undefined feedforward term is used in the present constant-reference experiments. To avoid windup while preserving a simple implementation,
\begin{equation}
\xi_{k+1}
=
\Pi_{\Xi}\!\left(\xi_k+T_f e_F(k)\right),
\label{eq:integral_proj}
\end{equation}
where $\Pi_{\Xi}$ denotes projection onto a predetermined integral-state interval $\Xi$.

The low-bandwidth disturbance estimate is updated from the measured one-step innovation,
\begin{equation}
\begin{aligned}
\hat d_{F,k+1}
&=(1-\beta_d)\hat d_{F,k} \\
&\quad+\beta_d\Big[
e_F(k+1)-\hat a e_F(k)-\hat b u_{n,k}
-\hat g^\top\vartheta_{j(k)}
\Big].
\end{aligned}
\label{eq:dist_est}
\end{equation}
with $0<\beta_d\le1$. Under the exact nominal scalar model, the bracketed term equals $d_{F,k}$ plus measurement noise. Model-parameter mismatch and disturbance-estimation error are therefore retained in the experimentally determined force-prediction bound.

\subsection{Recursive Multirate Prediction}

To keep the slow controller consistent with the implemented architecture, the $m$ fast normal commands are \emph{not} independent slow decision variables. Instead, for each scenario $s\in\mathcal P$, the nominal fast controller \eqref{eq:fast_control} is recursively simulated at the fast sampling rate for each candidate orientation sequence. Within the slow predictor, the disturbance estimate is held at its current value over the short horizon, and the integral projection is assumed inactive; the corresponding predicted integral state and command are explicitly constrained to remain within their admissible sets.

For each predicted fast step $h$,
\begin{align}
\hat u_{n,h}^{(s)}
&=-K_p\hat e_{F,h}^{(s)}-K_i\hat\xi_h^{(s)}
-\hat b^{-1}\hat g^\top\vartheta(h)
-\hat b^{-1}\hat d_{F,j},\nonumber\\
\hat e_{F,h+1}^{(s)}
&=a^{(s)}\hat e_{F,h}^{(s)}
+b^{(s)}\hat u_{n,h}^{(s)}
+g^{(s)\top}\vartheta(h)
+\hat d_{F,j},\nonumber\\
\hat\xi_{h+1}^{(s)}
&=\hat\xi_h^{(s)}+T_f\hat e_{F,h}^{(s)} .
\label{eq:recursive_force}
\end{align}
At each image interval, the predicted mean force error is computed using \eqref{eq:mean_force}, and the image state is propagated by \eqref{eq:image_model}. Because all recursions are affine in the candidate orientation increments while the predicted command and integral states remain inside their linear region, the resulting slow optimization remains a quadratic program (QP).

\subsection{Slow Image-Guided Orientation Program}

Over a horizon of $N$ image intervals, define
\begin{equation}
\Delta\Theta_j
=
\mathrm{col}
(\Delta\theta_{j|j},\ldots,\Delta\theta_{j+N-1|j}),
\label{eq:decision}
\end{equation}
with $\vartheta_{j-1|j}=\vartheta_{j-1}$ and
$\vartheta_{j+r|j}=\vartheta_{j+r-1|j}+\Delta\theta_{j+r|j}$.
The reconstructed image state \eqref{eq:image_recon} initializes the prediction.

The proposed controller solves the scenario-constrained QP. Receding-horizon optimization is attractive here because
state/input constraints can be incorporated directly into the
online control problem \cite{mayne2000constrained}; force-constrained optimization
has also been emphasized in recent robotic ultrasound \cite{duan2024safe}.
\begin{align}
\min_{\Delta\Theta_j}
&\sum_{s=1}^{N_p}\omega_s
\sum_{r=0}^{N-1}
\left(
\|\hat e_{I,j+r|j}^{(s)}\|_{W_I}^2
+q_F|\hat{\bar e}_{F,j+r|j}^{(s)}|^2
+\|\Delta\theta_{j+r|j}\|_R^2
\right)
\label{eq:slow_qp}\\
\text{s.t.}\quad
&F_{\min}+\varepsilon_{F,h}^{(s)}
\le \hat F_{n,h|j}^{(s)}
\le F_{\max}-\varepsilon_{F,h}^{(s)},\nonumber\\
&\hat u_{n,h|j}^{(s)}\in\mathcal U_n,\qquad
\hat\xi_{h|j}^{(s)}\in\Xi,\nonumber\\
&\theta_0+\vartheta_{j+r|j}\in\Theta,\qquad
\Delta\theta_{j+r|j}\in\Delta\Theta,\nonumber
\end{align}
for every retained scenario and every relevant fast sample $h$ in the horizon. Here $W_I\succeq0$, $q_F\ge0$, $R\succ0$, $\omega_s\ge0$, and $\sum_s\omega_s=1$; equal scenario weights are used unless otherwise justified. Image error is a performance variable rather than a hard safety variable. Only the first increment is applied. If the image is stale/invalid or the QP is infeasible, the last admissible orientation is held while the fast safety layer remains active.

Baseline B2 uses the same image feature and the same orientation and rate limits, but omits timestamp reconstruction and force-coupling prediction:
\begin{equation}
\Delta\theta_j^{B2}
=
\Pi_{\mathcal A_j}\!\left[-K_I e_I(\ell_j)\right],
\label{eq:B2}
\end{equation}
where $K_I\in\mathbb R^{n_\theta\times n_I}$ and
\[
\mathcal A_j=
\{\Delta\theta:
\Delta\theta\in\Delta\Theta,\;
\theta_0+\vartheta_{j-1}+\Delta\theta\in\Theta\}.
\]

\subsection{Sample-Wise Force Safety Filter}

The slow QP constrains nominal predicted trajectories, but an independent fast filter has priority at every force sample. For scenario $s$, define the one-step nominal force prediction under candidate command $u$:
\begin{equation}
\hat F_{n,k+1}^{(s)}(u)
=
F_d+a^{(s)}e_F(k)+b^{(s)}u
+g^{(s)\top}\vartheta_{j(k)}+\hat d_{F,k}.
\label{eq:one_step_force}
\end{equation}
The experimentally validated one-step error bound $\varepsilon_{F,1}^{(s)}$ includes model residual, disturbance-estimation error, and force-measurement uncertainty. The applied command is
\begin{align}
u_{n,k}
=\arg\min_{u\in\mathcal U_n}\, &(u-u^0_{n,k})^2
\label{eq:safety_filter}\\
\text{s.t.}\,
&F_{\min}+\varepsilon_{F,1}^{(s)}
\le\hat F_{n,k+1}^{(s)}(u)
\le F_{\max}-\varepsilon_{F,1}^{(s)}, \,\forall s .
\nonumber
\end{align}
For the scalar affine model, \eqref{eq:safety_filter} is a one-dimensional convex QP. If it is infeasible, force limits are not relaxed; the supervisor exits nominal operation and commands a predetermined controlled retraction.

\subsection{Local Analytical Properties}

Two modest local properties are used instead of a stronger coupled small-gain claim.

\textbf{Proposition 1 (nominal force-loop stability).}
Consider the unsaturated nominal PI force loop with the safety filter inactive, the integral projection inactive, and coupling/disturbance terms equal to their nominal compensated values. For scenario $s$, define
\begin{equation}
A_F^{(s)}
=
\begin{bmatrix}
a^{(s)}-b^{(s)}K_p & -b^{(s)}K_i\\
T_f & 1
\end{bmatrix}.
\label{eq:AF}
\end{equation}
If there exist $P_F=P_F^\top\succ0$ and $Q_F=Q_F^\top\succ0$ such that
\begin{equation}
A_F^{(s)\top}P_FA_F^{(s)}-P_F\preceq-Q_F,
\qquad s=1,\ldots,N_p,
\label{eq:lyap}
\end{equation}
then the nominal force loop is uniformly exponentially stable for every accepted model in the bank. Bounded coupling mismatch, disturbance-estimation error, and model residuals act as bounded inputs to this locally stable loop.

\textbf{Proposition 2 (force-interval preservation).}
Suppose $F_n(k)\in[F_{\min},F_{\max}]$, the true one-step force lies within $\varepsilon_{F,1}^{(s)}$ of at least one accepted scenario, and \eqref{eq:safety_filter} is feasible. Then its tightened constraints imply
\[
F_n(k+1)\in[F_{\min},F_{\max}].
\]
By induction, the interval is invariant during maintained-contact operation while the filter remains feasible and the model-coverage assumptions hold. Supervisory retraction intentionally terminates this maintained-contact mode and is not part of the invariance claim.

No recursive-feasibility guarantee is claimed for the slow QP because no terminal invariant set or equivalent mechanism is imposed. The theory is therefore deliberately local: \eqref{eq:lyap} provides a checkable nominal force-loop condition, while \eqref{eq:safety_filter} provides an independently checkable force-protection condition.

\begin{figure}[t]
\centering
\fbox{\parbox[c][0.92in][c]{0.94\columnwidth}{\centering
\textbf{Dual-rate architecture figure placeholder}\\
slow image: timestamp reconstruction $\rightarrow$ scenario QP $\rightarrow$ held orientation\\
fast loop: wrench $\rightarrow$ force PI/disturbance compensation $\rightarrow$ safety filter\\
supervisor: force/moment, image validity, workspace, sensing, communication, retraction}}
\caption{Dual-rate control architecture and supervisory hierarchy.}
\label{fig:architecture}
\end{figure}


==> sections_v2/05_validation_results.tex <==
\section{Experimental Validation}
\label{sec:validation}

\subsection{Protocol and Metrics}
Validation was organized to separate estimator accuracy, dynamic force regulation, image-guided scanning, and feasibility on living tissue. All controller parameters, image-validity thresholds, force limits, and model-selection rules were frozen before comparative testing. The nominal contact-force target was $F_d=10.0$~N for the dynamic and image-guided experiments. Quantitative analyses used complete trials as the experimental units; high-rate force samples and ultrasound frames within a trial were not treated as independent replicates.

Four validation cases were considered. First, static phantom tests compared the probe-normal force regulation with various levels of reference at commanded loads of 10, 15, and 20~N, with \textcolor{red}{3 repetitions per load; confirm final number}. Second, dynamic phantom tests imposed repeatable surface motion with independently measured geometry to evaluate force tracking under controlled disturbance. Third, an image-guided scan used a vessel-mimicking channel of known path to evaluate the interaction between force regulation and image-based lateral correction. The scan used $F_d=10.0$~N, a nominal scan velocity of 3~mm/s, and \textcolor{red}{5-mm initial lateral offset; confirm final protocol}. Finally, a popliteal-vessel scan was used as a secondary feasibility test on living tissue; these data were not pooled with phantom statistics.

The primary force-control outcome was trial-level
\begin{equation}
{\rm RMSE}_F=
\sqrt{\frac{1}{|\mathcal K|}
\sum_{k\in\mathcal K}\left(F_d-F_n(k)\right)^2},
\label{eq:rmseF_exp}
\end{equation}
computed after the specified settling interval. For image-guided scanning, the primary image outcome was lateral centering error,
\begin{equation}
{\rm RMSE}_y=
\sqrt{\frac{1}{|\mathcal K_I|}
\sum_{j\in\mathcal K_I}e_y^2(j)},
\label{eq:rmsey_exp}
\end{equation}
reported both from the in-loop image estimate and, when available, from independently registered vessel-path ground truth. Secondary outcomes were peak force error, lateral settling time, fraction of valid ultrasound frames, longest invalid-frame run, alignment excursion, contact-loss/safety events, and computation/timing statistics. Controller effects should be reported as paired trial-level differences with 95\% confidence intervals; \textcolor{red}{add block/site random effect only if the final number of independent blocks supports it}.

\subsection{Static and Dynamic Phantom Validation}

The static phantom test establishes the accuracy and repeatability of the force signal used by the controller. For each applied load, the mean estimated force, within-load standard deviation, and estimation error should be reported. Because the current regulator includes updated probe-frame transformation and compensation terms, the static sweep should be collected using the same frozen software build used for the controller experiments. A linear fit,
$\hat F_n=a_F F_{\rm ref}+b_F$, may be reported to separate multiplicative scale error from additive offset. \textcolor{red}{The final manuscript should include force-tracking RMSE or MAE, and within-/across-session repeatability}.

The dynamic phantom test evaluates force tracking when the local surface moves relative to the probe. Surface displacement is prescribed by \textcolor{red}{rotating-stage/actuator geometry and motion frequencies} and measured independently. Because no independent force transducer is available during motion, dynamic RMSE is interpreted as tracking error in the controller's force space, together with the static accuracy bound above. Across \textcolor{red}{$N$ trials at each motion condition}, the proposed controller achieved \textcolor{red}{XXX force RMSE}, \textcolor{red}{XXX peak error}, and \textcolor{red}{XXX contact-loss count}. Fig.~\ref{fig:exp_results}(a) shows representative synchronized surface motion and force tracking, while Table~\ref{tab:validation_summary} summarizes trial-level outcomes.

\subsection{Image-Guided Scan and Ablation}

The image-guided phantom scan evaluates whether image-based correction can reduce lateral vessel-centering error without degrading contact-force regulation. The phantom vessel path should be registered to the robot base frame so that image-derived centering error can be compared with an independent geometric reference. Over the analysis window beginning \textcolor{red}{$T_s$ s after touchdown}, the full controller is compared with \textcolor{red}{the final ablation set actually implemented; e.g., image correction disabled, P-only, PI, and/or the Section-IV B1/B2/P variants}. Only one control component should be changed at a time, with common force, velocity, orientation, and safety limits across conditions.

The final comparison should report \textcolor{red}{${XXX RMSE}_y$}, ground-truth lateral RMSE, lateral settling time, \textcolor{red}{${RMSE}_F$}, maximum force error, valid-frame fraction, and longest stale-image interval. The central paper claim should be supported only if the complete controller \textcolor{red}{reduces lateral/image error relative to the force-only or decoupled baseline while maintaining or improving force RMSE and peak force}. If the Section-IV B1/B2/P controller comparison is retained, the final results must explicitly report B2--B1 (benefit of image feedback) and P--B2 (benefit of delay/coupling compensation); otherwise, those claims should be removed from the Abstract and Introduction.

\begin{table}[t]
\caption{Experimental validation summary. Replace highlighted entries with frozen trial-level results.}
\label{tab:validation_summary}
\centering
\footnotesize
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{p{0.35\columnwidth}p{0.26\columnwidth}p{0.28\columnwidth}}
\toprule
Validation case & Primary metric & Result \\
\midrule
Static phantom & Force-estimation error & \textcolor{red}{RMSE/MAE; $a_F,b_F$} \\
Dynamic phantom & Force RMSE / peak error & \textcolor{red}{values; 95\% CI} \\
Image-guided scan & Lateral RMSE / force RMSE & \textcolor{red}{values; 95\% CI} \\
Image availability & Valid frames / max stale run & \textcolor{red}{\% / frames} \\
Real-time execution & Loop and image timing & \textcolor{red}{mean, p99/max, latency} \\
Human feasibility & Force/lateral/safety outcomes & \textcolor{red}{values} \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[t]
\centering
\fbox{\parbox[c][1.00in][c]{0.94\columnwidth}{
\centering
\textbf{FINAL FIGURE PLACEHOLDER}\\
(a) dynamic-phantom surface motion and force tracking;\\
(b) image-guided scan: $e_y$, $F_n$, and controller command;\\
(c) trial-level force RMSE; (d) lateral RMSE / ablation result.
}}
\caption{Experimental validation. Quantitative metrics are computed from synchronized raw logs; any filtering shown in representative traces is for visualization only.}
\label{fig:exp_results}
\end{figure}

\subsection{Volunteer-Tissue Feasibility}

A single-subject popliteal scan was used to examine whether the frozen controller could operate on living tissue with compliance, curvature, and involuntary motion not represented by the phantom. No independent force ground truth was available; therefore, this test is interpreted only as feasibility. \textcolor{red}{Reported quantities should include force RMSE relative to the commanded setpoint, peak force, lateral centering RMSE, valid-frame fraction, longest invalid-frame run, maximum alignment excursion, contact-loss/safety events, and scan duration.} The final values are \textcolor{red}{insert volunteer results}. Given that the reported data were from only the feasibility study on living human tissue, they should not be used to claim clinical accuracy or subject-level generalization.



==> sections_v2/06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
The contribution is explicit control of \emph{multirate coupling}, not the first combination of image and force feedback. Prior work already establishes image servoing, force/orientation regulation, and image-dependent force adaptation \cite{jiang2020normal,jiang2021force,akbari2021,zakeri2025,piedra2026}. Here, P--B2 tests the value of predicting the force consequence of an orientation update before the corresponding image arrives, whereas B2--B1 tests image feedback itself. The ablations, therefore, guard against a misleading trade-off in which image error improves only by accepting larger force excursions, or vice versa.

The implementation is explicitly multirate. The safety-relevant contact loop operates near 1~kHz, whereas ultrasound acquisition and image processing are substantially slower; the experimental report also identifies a still slower orientation-alignment loop. This separation is useful because image delay or a dropped frame should degrade guidance rather than disable contact regulation. At the same time, the slower correction loops can move the robot configuration and therefore perturb the estimated normal force. The final ablation should determine whether those cross-loop effects are sufficiently large to justify the model-informed coordination proposed in Section~IV. 

Several limitations should remain explicit. First, dynamic force tracking is evaluated in the estimate space and inherits the accuracy and repeatability limits established by the static phantom calibration. Second, stale-image handling, lateral-command saturation, and consistent derivative/integral time bases must be finalized before the controller ablation, because otherwise the comparison would confound algorithmic effects with implementation defects. Finally, the human experiment is a single-subject feasibility demonstration and cannot establish clinical safety, anatomical generalization, or diagnostic image quality. Broader translation will require independent image-validation data, additional subjects and anatomies, and re-evaluation of timing and uncertainty bounds across scanners and probe configurations.

==> sections_v2/07_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This paper addresses robotic ultrasound as a multirate interaction-control problem in which high-rate contact regulation is coupled to slower probe-alignment and image-guided corrections. The proposed framework combines local force--pose--image modeling, high-rate force regulation, constrained slower-loop updates, and an image-independent safety path. Validation is organized from independent static force calibration to dynamic phantom tracking, image-guided scanning, and secondary volunteer-tissue feasibility. The final experiments show \textcolor{red}{insert primary force result} together with \textcolor{red}{insert primary image/lateral result and safety result}. These findings \textcolor{red}{support / do not yet support} the benefit of explicitly coordinating the force and image loops under the tested conditions. Claims are restricted to the validated force, motion, orientation, imaging, tissue, and timing ranges.

\section*{Acknowledgment}
The authors acknowledge support from The University of Alabama faculty startup fund and the Alabama Transportation Institute. This work was also supported by the U.S. Department of Transportation University Transportation Centers Program through CR2C2, Grant No.~69A3552348304.


==> sections_v3/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Brightness mode (B-mode) ultrasound provides real-time, radiation-free imaging with comparatively low cost, but its image quality is strongly coupled to how the probe interacts with the tissue. During manual scanning, a sonographer continuously
coordinates probe position and orientation with contact force while responding to local surface geometry, tissue compliance, and the observed ultrasound image. Robotic ultrasound, therefore, presents a coupled sensing-and-control problem rather than a conventional trajectory-following task. Existing reviews accordingly identify scanning-path generation, probe-tissue force regulation, and image-quality or orientation optimization as central components of autonomous robotic ultrasound systems \cite{li2021overview,haxthausen2021,salcudean2022,jiang2023review}. More recent surveys note two remaining limitations that are particularly relevant from a control perspective: interaction wrench components associated with probe orientation are often simplified, and real-time ultrasound feedback remains less commonly integrated into online scan optimization \cite{bi2024,munir2025,han2025clinical}. 
% These limitations motivate control architectures in which the probe-tissue dynamics, cross-coupling between controlled variables, and heterogeneous sensing rates are treated explicitly. 

Early image-guided robotic ultrasound demonstrated that features extracted directly from ultrasound images can close the robot-positioning loop \cite{abolmaesumi2002}. Subsequent visual-servoing approaches optimized ultrasound confidence measures to improve acoustic coupling and probe orientation \cite{chatelain2015}. In parallel, interaction-force information has been exploited for estimating the local surface normal and regulating probe orientation \cite{jiang2020normal,jiang2021force,ma2022asee}. More recent explicit force-control strategies directly regulate contact forces and moments to achieve responsive probe - tissue interaction under heterogeneous and dynamic conditions \cite{piedra2026}. Ultrasound feedback has also enabled autonomous entering and alignment of tubular structures \cite{jiang2022tubular}, while image-quality estimated have been used to adapt the commanded contact force rather than maintaining a fixed force across different imaging conditions \cite{akbari2021,zakeri2025}. Collectively, these studies establish that image and force sensing provide complementary information. Consequently, simply combining the two feedback modalities is no longer, by itself, sufficient to contribute to control. 

Learning-based approaches have further expanded the achievable level of autonomy. Deep reinforcement learning has been used to navigate toward anatomical targets from ultrasound observations \cite{hase2020}; reinforcement learning policies have combined visual scene perception with compliant force control for scanning moving, markerless targets \cite{ning2021rl}; and inverse reinforcement learning has transferred active-compliance behavior to uncertain soft environments \cite{ning2024irl}. Constraint-aware policy optimization explicitly incorporates interaction-force limits during policy learning \cite{duan2025safe}, while recent large-scale imitation learning has demonstrated substantial generalization across an autonomous carotid-ultrasound workflow \cite{jiang2025ultrabot}. These developments demonstrate the potential of learning for perception, decision making, and reference generation. At the same time, recent reviews emphasize limitations associated with medical-data availability, domain variation, and insufficient incorporation of physical knowledge \cite{bi2024,yip2023}. For contact-rich medical robotics, this suggests a useful separation of roles: learned perception can provide task-relevant image information, whereas the high-bandwidth interaction loop should retain sufficient physical structure to support constraint enforcement, robustness analysis, and failure detection. 

A control issue that is less explicitly addressed in this literature is the multirate dynamic coupling between force regulation and image-guided probe correction. Robot state and wrench measurements can be updated at high rates, whereas B-mode images are acquired, transferred, and processed at substantially lower rates and with non-negligible latency. This mismatch has already appeared in practical robotic ultrasound implementations; for example, image-based force adjustment has been implemented with a slower image-quality loop than the underlying robot-control loop \cite{akbari2021}. The difficulty is more fundamental than asynchronous sensing alone. An orientation correction computed from an image changes probe indentation, the contact moment, and consequently the normal force before a new image measurement becomes available. Conversely, a fast force regulator reacts to the normal displacement induced by the orientation update and can partially oppose the intended image-based correction. Tissue stiffness, local curvature, surface motion, and uncertainty in image sensitivity further modify this bidirectional interaction. Recent dual-loop approaches have demonstrated image-dependent force adaptation and robust contact-force tracking \cite{zakeri2025}, while explicit force/moment regulation improves dynamic interaction performance \cite{piedra2026}. In addition, Li et al. \cite{li2026trajectory} explicitly incorporate trajectory-dependent feedforward and delay compensation for dynamic contact-force tracking, and Qian et al. \cite{qian2026symmetry} combine image guidance with biomechanics-informed force estimation/control. However, these advances do not directly formulate the image-guided orientation loop and the high-rate force loop as an identified, delayed multirate system whose cross-coupling can be predicted and incorporated into controller design. 


This paper treats that coupling as the control problem itself. We propose a
dual-rate orientation controller in which the slow image-guided loop is made
aware of both its own latency and its effect on the fast contact loop: the
alignment error is reconstructed to the present instant from the frame's
capture timestamp, the force consequence of a candidate correction is predicted
from an orientation-to-force coupling conditioned on the image cue, and the
prediction credits the fast loop with the portion of that disturbance it will
reject before the next frame arrives. The last term is what separates the
method from a one-step safety filter, which must assume the disturbance
persists and therefore throttles the correction more than necessary.

The controller is demonstrated on a platform with \emph{no force/torque
sensor}, with contact force estimated from joint torques. This configuration is
attractive for cost, cabling, and sterilization and is increasingly common on
collaborative arms, but it raises the force noise floor and introduces
model-dependent bias, which sharpens every trade-off the controller must make.
The contributions are:

\vspace{-0.5 mm}
\begin{enumerate}
    \item a dual-rate orientation controller combining timestamp-based delay
    reconstruction, prediction of the orientation-to-force coupling conditioned
    on the image cue, and explicit crediting of the fast loop's disturbance
    rejection over the frame interval;

    \item the design condition, relating the coupling, the rotation limit, and
    the force-loop rejection rate, that determines whether the predictive
    constraint modifies the commanded correction, together with the
    identification of that coupling against known probe angle; and

    \item hardware evaluation against force-only and newest-frame baselines
    under phantom contact, with ablations separating the predictive barrier's
    contribution from a fixed-rate alternative and from online parameter
    adaptation, and a volunteer popliteal scan.
\end{enumerate}

==> sections_v3/02_system.tex <==
\section{System and Sensorless Force Estimation}
\label{sec:system}

\subsection{Platform}
The platform is a Kinova Gen3 six-degree-of-freedom manipulator carrying a
Telemed Artus linear probe in a rigid printed holder. No force/torque sensor is
present; the contact wrench is estimated from the torque sensors integrated in
each actuator. This removes the cost, cabling, and sterilization burden of a
wrist-mounted transducer at the expense of a higher noise floor and a
model-dependent bias, and it constrains the orientation controller developed in
Section~\ref{sec:control} in ways quantified below.

The arm is commanded in joint position at $f_f=1$~kHz through the
manufacturer's low-level cyclic interface. A Cartesian velocity command
$v_c\in\mathbb R^{6}$ is mapped to joint rates through a damped least-squares
inverse of the geometric Jacobian and integrated to the streamed position
command,
\begin{equation}
\dot q_c=J^{\dagger}(q)\,v_c,\qquad
q_c^{k+1}=q_c^{k}+\dot q_c\,\Delta t_f,
\label{eq:intcmd}
\end{equation}
with $\Delta t_f=1/f_f$ and $\dot q_c$ scaled uniformly when any joint exceeds
its rate limit. B-mode frames are captured from the scanner display at
$f_I\approx30$~Hz. Acquisition-to-use latency is dominated by the
confidence-map solve quantified in Section~\ref{sec:sensing} and by the
scanner's own acquisition-to-display delay, which is internal to the device and
was not independently measured here. The controller of
Section~\ref{sec:control} therefore compensates delay from each frame's own
capture timestamp rather than from an assumed constant.

\subsection{Wrench Estimation from Joint Torques}
Let $q\in\mathbb R^{6}$ denote measured joint coordinates and
$\tau_m\in\mathbb R^{6}$ measured joint torques. The rigid-body model is
\begin{equation}
M(q)\ddot q+C(q,\dot q)\dot q+g(q)+\tau_{f}=\tau_m+J^{\!\top}(q)\,h_c ,
\label{eq:dyn}
\end{equation}
with $h_c$ the contact wrench at the tool. Probe motion during scanning is slow
(below $0.02$~m/s); at these rates the inertial and Coriolis terms are smaller
than the torque measurement noise, and the velocity feedback available from the
actuators is already a numerical derivative whose further differentiation would
amplify that noise quadratically. Both terms are therefore dropped and the
gravity torque is evaluated by a quasi-static recursive Newton--Euler pass,
\begin{equation}
\tau_g(q)=\mathrm{RNEA}\bigl(q,\dot q=0,\ddot q=0\bigr),
\label{eq:rnea}
\end{equation}
which for link $i$ with rotation ${}^{i}\!R_{i-1}$, center of mass $c_i$, and
mass $m_i$ reduces to the outward propagation of the gravitational
acceleration and the inward propagation of forces and moments,
\begin{align}
{}^{i}a_i &= {}^{i}\!R_{i-1}\,{}^{i-1}a_{i-1}, \nonumber\\
{}^{i}f_i &= {}^{i}\!R_{i+1}\,{}^{i+1}f_{i+1}+m_i\,{}^{i}a_i, \nonumber\\
{}^{i}n_i &= {}^{i}\!R_{i+1}\,{}^{i+1}n_{i+1}
  + c_i\times m_i\,{}^{i}a_i \nonumber\\
  &\quad + p_{i+1}\times {}^{i}\!R_{i+1}\,{}^{i+1}f_{i+1},
\label{eq:rneaprop}
\end{align}
with ${}^{0}a_0=-g_w$ and $\tau_{g,i}={}^{i}n_i^{\!\top}z_i$. Link parameters
are taken from the manufacturer's URDF, with the bracelet-link mass and center
of mass updated for the probe and holder.

Strain-wave gearing introduces a position-periodic transmission error that
appears as a torque ripple of the same order as the contact signal. It is
modeled per joint as a direction-dependent harmonic term $\tau_{te}(q)$
identified offline from free-space pose sweeps. The estimated contact wrench is
\begin{equation}
\hat h_c=\bigl(J^{\!\top}(q)\bigr)^{\!+}
\bigl(\tau_f-\tau_g(q)-\tau_{te}(q)\bigr)-h_0 ,
\label{eq:wrench}
\end{equation}
where $\tau_f$ is $\tau_m$ after a per-joint second-order Butterworth filter
with a $25$~Hz cutoff at $1$~kHz, $(\cdot)^{+}$ denotes the pseudoinverse, and
$h_0\in\mathbb R^{6}$ is a free-space tare acquired while the arm holds
position immediately before contact. Because $h_0$ absorbs whatever residual
the model leaves at that pose, it is preceded by a conditioning motion that
walks each joint against and then along its press direction, so that the tare
is taken on the same branch of each joint's friction loop that the subsequent
press will traverse.

The regulated variable is the probe-axis component of the estimated contact
force, expressed in a probe frame whose origin is the acoustic face,
\begin{equation}
F_n=-\,e_3^{\!\top}\,{}^{P}\!R_B\,\hat F_c ,
\label{eq:fn}
\end{equation}
where ${}^{P}\!R_B$ is the base-to-probe rotation, $e_3$ selects the beam axis,
and the leading sign makes compression positive, the beam axis being directed
out of the acoustic face. Referencing the probe frame to the face rather than
to the flange is required for the moment channel and for the orientation
commands of Section~\ref{sec:control}; the measured offset along the probe axis
is $72$~mm.

\subsection{Achievable Accuracy}
Since \eqref{eq:wrench} admits no independent force reference during operation,
its accuracy bounds every downstream claim. Static loading against a reference
scale over $5$--$20$~N gives a mean absolute error of $1.90$~N, or $25.2\%$ of
the commanded level. That average understates the structure of the error: the
estimate reads high at low commanded force, by $57.9\%$ at $5$~N and $36.9\%$
at $8$~N, and the discrepancy falls monotonically to $0.3\%$ at $20$~N. This is
the signature of a residual that is roughly fixed in absolute terms and
therefore becomes negligible as the contact signal grows, consistent with the
ripple behavior reported below. The figures come from a single loading run and
bound the estimate rather than calibrate it.
Table~\ref{tab:te} reports the within-dwell
standard deviation of the force error with and without the transmission-error
term; compensation reduces the error at every level tested, with diminishing
relative benefit as the contact signal grows relative to the ripple.

\begin{table}[t]
\caption{Force-error standard deviation per dwell (N) with and without
transmission-error compensation.}
\label{tab:te}
\centering
\footnotesize
\begin{tabular}{cccc}
\toprule
$F_d$ (N) & TE on & TE off & reduction \\
\midrule
 5 & 0.299 & 0.421 & 29\% \\
 8 & 0.249 & 0.336 & 26\% \\
10 & 0.185 & 0.232 & 20\% \\
15 & 0.499 & 0.530 &  6\% \\
20 & 0.560 & 0.624 & 10\% \\
\bottomrule
\end{tabular}
\end{table}


==> sections_v3/03_sensing.tex <==
\section{Orientation Sensing from Ultrasound}
\label{sec:sensing}

\subsection{Alignment Cues}
When the probe deviates from the local surface normal, one end of the array
lifts, acoustic coupling degrades on that side, and image quality falls off
from the transducer face downward. We evaluate three scalar cues for this
asymmetry, written in a common normalized form so that the controller of
Section~\ref{sec:control} is independent of which is selected. Throughout,
$I$ denotes the selected cue and is dimensionless, with $I=0$ corresponding to
a laterally symmetric image.

\subsection{Near-Field Intensity Imbalance}
The least expensive cue compares mean gray level between the left and right
halves of the near field. With $\bar g_L$ and $\bar g_R$ the mean intensity
over the corresponding regions of the upper portion of the image,
\begin{equation}
I_{\rm prox}=\frac{\bar g_L-\bar g_R}{\bar g_L+\bar g_R}.
\label{eq:proxy}
\end{equation}
Its principal limitation is that it does not distinguish degraded coupling from
hypoechoic anatomy: a vessel lying off-center darkens one side and is
indistinguishable from misalignment.

\subsection{Random-Walk Confidence Map}
A physically motivated alternative is the ultrasound confidence map of
Karamalis \emph{et al.}~\cite{karamalis2012}, which assigns to each pixel the
probability that a random walker released there reaches the transducer before
the far field, with edge weights derived from intensity gradients under an
attenuation model. Writing $c(r,\kappa)\in[0,1]$ for the confidence at row $r$
and column $\kappa$, the map is obtained by solving a sparse Dirichlet problem
on the pixel graph. We solve it at $96\times96$ by direct factorization, with
the symbolic analysis performed once. The full per-frame cost on the
experimental hardware -- crop, resize, solve, and feature extraction -- was
$17.2\pm7.0$~ms over $\approx1400$ frames of phantom and volunteer operation,
under half the $33$~ms frame budget on average, with occasional solves
approaching it. The solve runs on a dedicated thread, and each result is
tagged with the capture timestamp of the frame from which it was computed,
which Section~\ref{sec:control} requires.

Two cues are extracted. The first applies \eqref{eq:proxy} to confidence rather
than intensity,
\begin{equation}
I_{\rm cm}=\frac{\bar c_L-\bar c_R}{\bar c_L+\bar c_R},
\label{eq:cmimb}
\end{equation}
with $\bar c_L$ and $\bar c_R$ the mean confidence over the left and right
halves. The second uses the depth at which confidence falls below a threshold
$c_{\rm th}$,
\begin{equation}
d(\kappa)=\frac{1}{N_r-1}\min\{\,r:\;c(r,\kappa)<c_{\rm th}\,\},
\label{eq:cdepth}
\end{equation}
and takes its least-squares slope against normalized lateral position
$x_\kappa\in[-1,1]$, negated so that a more confident left side yields a
positive value:
\begin{equation}
I_{\rm slope}=-\,\Bigl(\textstyle\sum_\kappa x_\kappa d(\kappa)\Bigr)
\Bigl/\Bigl(\textstyle\sum_\kappa x_\kappa^{2}\Bigr).
\label{eq:cslope}
\end{equation}
Unlike \eqref{eq:proxy} and \eqref{eq:cmimb}, \eqref{eq:cslope} depends on the
depth at which the reliable region terminates rather than on its magnitude, so
a spatially uniform change in gain or in overall confidence leaves it
unchanged.

Map parameters were selected offline on recorded scans: $\alpha=2.0$,
$\beta=10.0$, $\gamma=0.05$, and $c_{\rm th}=0.5$, the threshold chosen so that
the confident-depth boundary of \eqref{eq:cdepth} falls near mid-depth of the
image over the range of coupling encountered, where it is most sensitive to
asymmetry.

\subsection{Noise Floors}
Because the three cues enter an identical control law, the relevant figure of
merit is sensitivity per unit angle divided by noise rather than sensitivity
alone. Single-frame noise was estimated over $468$ frames of steady contact as
the standard deviation of the frame-to-frame difference divided by $\sqrt2$,
giving $1.95\times10^{-3}$ for $I_{\rm prox}$, $4.25\times10^{-3}$ for
$I_{\rm cm}$, and $5.73\times10^{-3}$ for $I_{\rm slope}$. The confidence cues
are thus $2.2\times$ and $2.9\times$ noisier than the intensity imbalance and
must exceed those factors in angular sensitivity to be preferred.
Section~\ref{sec:char} evaluates this against known probe angle.
\tbd{re-verify these three noise floors against the final cue configuration
before submission}


==> sections_v3/04_control.tex <==
\section{Dual-Rate Control}
\label{sec:control}
\begin{figure*}[t]
  \centering
  \input{figures/architecture_diagram}
  \caption{Dual-rate control architecture diagram. The 30 Hz image loop reconstructs delay and scales orientation commands via a predictive barrier, while the 1 kHz force loop regulates contact force using sensorless wrench estimation.}
  \label{fig:control_architecture}
\end{figure*}
\subsection{Fast Force Loop}
The inner loop regulates $F_n$ to a constant reference $F_d$ by commanding
probe-axis velocity at $1$~kHz,
\begin{equation}
v_n=K_p e_F+K_i\!\int\! e_F\,dt-K_d\dot{\hat F}_n,
\qquad e_F=F_d-F_n,
\label{eq:pid}
\end{equation}
with $v_n$ saturated and integral accumulation gated on established contact.
Gains were tuned at the operating force used throughout and held fixed across
every reported condition.
For the purposes of the orientation controller, the closed force loop is
characterized by its first-order disturbance-rejection rate
\begin{equation}
a=K K_p ,
\label{eq:arate}
\end{equation}
where $K$ is the local contact stiffness. On the phantom of
Section~\ref{sec:char},
$K=2065$~N/m and $K_p=6.25\times10^{-3}$, giving
$a\approx12.9~\mathrm{s^{-1}}$.

\subsection{Orientation Channel}
The outer loop rotates the probe about the in-plane axis of its face so as to
drive the selected cue to zero,
\begin{equation}
\omega=-K_I\,\sigma\,I,\qquad
\sigma=\operatorname{sign}\!\left(\partial I/\partial\theta\right),
\label{eq:imglaw}
\end{equation}
with $\omega$ saturated at $\omega_{\max}$ and constrained by a limit on net
angular excursion measured from the touchdown orientation. The excursion limit
is enforced directionally: beyond it, rotation that would increase the
excursion is suppressed while rotation returning toward the touchdown
orientation is permitted, so that the limit bounds departure without
preventing recovery. Since the Jacobian
references the interface origin rather than the acoustic face, the commanded
angular rate is accompanied by $-\,\omega\times d$ on the linear rows, with $d$
the origin-to-face offset, so that the face rotates about itself rather than
translating.

A lateral asymmetry cue presupposes that the aperture is substantially
coupled: if contact is lost across a large fraction of the face, the cue
remains well defined but no longer reports misalignment. This is a limitation
of the cue rather than a condition the controller detects and handles
separately; the excursion limit above bounds how far a misreported cue can
drive the probe, and Section~\ref{sec:discussion} returns to the consequences.

The control law in \eqref{eq:imglaw} operates directly on the cue and requires
no conversion to angular units. Two model quantities, both expressed per unit
angle, are nevertheless required by the predictive terms below. The first is
the cue sensitivity
\begin{equation}
S=\frac{\partial I}{\partial\theta},
\label{eq:Sdef}
\end{equation}
which converts elapsed rotation into an equivalent change in the cue. The
second is the orientation-to-force coupling
\begin{equation}
g_\theta=\left.\frac{\partial F_n}{\partial\theta}\right|_{\delta},
\label{eq:gtheta}
\end{equation}
evaluated at fixed indentation $\delta$, which converts a candidate rotation
into a predicted force excursion. For a planar face pivoting about its own
center, tilting unloads one side of the contact patch to the same extent that
it loads the other, so $g_\theta$ is expected to remain small until an edge
leaves the surface, after which the cancellation fails. Since $|I|$ increases
as that unloading progresses, we adopt the affine parameterization
\begin{equation}
g_\theta(I)=g_0+g_1 I ,
\label{eq:gmodel}
\end{equation}
which reduces to a constant coupling when $g_1=0$. On the phantom reported
here the cue-dependent term was not resolvable from the constant one
(Section~\ref{sec:paramest}); the parameterization is retained because the
identification of Section~\ref{sec:char} shows the coupling itself to be
strongly regime-dependent across lift-off.
Both $S$ and $g_\theta$ may be estimated online by recursive least
squares with forgetting, a sign constraint inherited from calibration, and an
excitation gate suppressing updates in the absence of appreciable rotation;
Section~\ref{sec:results} reports results with the estimators active and with
them held at calibrated values.

\subsection{Three Controllers}
Three orientation policies are compared against an identical inner loop,
identical actuator and excursion limits, and an identical cue.

\textbf{B1} applies no orientation correction, $\omega\equiv0$.

\textbf{B2} applies \eqref{eq:imglaw} to the most recent available cue and
holds the resulting rate until the next frame, with no delay compensation and
no force prediction.

\textbf{P} adds two terms. The first is \emph{delay reconstruction}. The cue
was measured at capture time $t^c$ and the probe has rotated since, so the
controller acts on
\begin{equation}
\hat I(t)=I(t^c)+S\bigl(\theta(t)-\theta(t^c)\bigr),
\label{eq:recon}
\end{equation}
with $\theta$ retrieved from a $1$~kHz history buffer indexed by the frame's
own capture timestamp. The second is \emph{coupling prediction with fast-loop
simulation}. Over a horizon $T_h$ that spans one frame interval plus latency, the
controller integrates the predicted closed-loop response
\begin{equation}
\dot e_F=-a\,e_F+g_\theta(\hat I)\,\omega,\qquad
\dot{\hat I}=S\,\omega,
\label{eq:predsim}
\end{equation}
and selects a scale $s\in[0,1]$ on the commanded rate subject to $F_n$
remaining within $[F_d-\Delta F,\,F_d+\Delta F]$ over the horizon. Writing
$u(s)\in[0,1)$ for the predicted worst-case excursion normalized by the
admissible margin, $s$ is obtained as
\begin{equation}
s=\arg\min_{s\in[0,1]}\;(1-s)^2-\mu\log\!\bigl(1-u(s)^2\bigr).
\label{eq:barrier}
\end{equation}
The first term penalizes withholding correction and the second is a
logarithmic barrier on the force specification: it is negligible while the
predicted excursion is small, so $s\to1$ when the correction is harmless, and
diverges as the prediction approaches the admissible margin, so no minimizer
can select an infeasible command. The bound of a one-step filter is therefore
retained exactly, while $s$ varies continuously with the prediction rather
than switching at the boundary, which matters because the prediction inherits
the frame-to-frame variability of the image cue. Taking $\mu\to0$ recovers the
hard bound, and both are evaluated in Section~\ref{sec:results}. The term
$-a e_F$ is what distinguishes the proposed controller from a one-step
constraint: because the inner loop rejects part of the disturbance within the
frame interval, the predicted residual excursion is smaller and the correction
need not be throttled as severely. Setting $a=0$ recovers the one-step
constraint and is retained as an ablation.

\subsection{Activity of the Predictive Constraint}
Under saturated rotation, the quasi-static solution of \eqref{eq:predsim} gives
the steady force excursion
\begin{equation}
|e_F|_{\rm ss}\approx\frac{g_\theta\,\omega_{\max}}{a},
\label{eq:binding}
\end{equation}
so the constraint in P modifies the commanded rate only when
\begin{equation}
g_\theta\,\omega_{\max}\;\gtrsim\;a\,\Delta F .
\label{eq:bindcond}
\end{equation}
Equation~\eqref{eq:bindcond} is the design inequality for this architecture and
can be evaluated before experiments rather than inferred from them. It states
that a fast inner loop, a slow rotation limit, or a wide admissible band each
render the prediction inactive, in which case P reduces to B2 by construction.
Conversely, the prediction is consequential when the coupling is large, the
rotation limit is permissive, or the force tolerance is tight. Since $a=KK_p$,
the same inequality indicates that compliant tools, reduced contact gains, and
lower-bandwidth or noisier force channels all enlarge the regime in which the
architecture is warranted. Section~\ref{sec:results} selects
$\omega_{\max}=0.6$~rad/s and $\Delta F=0.5$~N on this basis
and reports the realized constraint
scale $s$ directly, so that the comparison is not presented at an operating
point where the constraint was never active.

==> sections_v3/05_characterization.tex <==
\section{Characterization Experiments}
\label{sec:char}

Characterization used a planar gelatin phantom prepared from $545$~g water,
$61$~g gelatin, and $7$~g cornstarch as a speckle agent, with acoustic coupling
gel at the interface. Scanner gain, dynamic range, time-gain compensation,
speckle reduction, and adaptive gain were fixed for all runs reported here; the
image cues of Section~\ref{sec:sensing} are comparable only within a fixed
display configuration.

\subsection{Contact Stiffness}
A force sweep at $\{5,8,10,15,20\}$~N with the probe stationary relates contact
force to face displacement, the latter obtained by forward kinematics on the
measured joint angles. A linear fit yields $K=2065$~N/m with $R^2=0.992$.
Incremental stiffness between adjacent levels ranges from $1757$ to
$2906$~N/m, a spread consistent with the nonlinear compression of gelatin over
this range and with time-dependent relaxation under sustained load; the
single-slope value is used throughout as a local linearization. At $F_d=15$~N
the corresponding indentation is $4.9$~mm, which for a face half-length of
$40$~mm predicts trailing-edge lift-off near $7^\circ$.

\subsection{Tilt Sweep}
With the orientation loop disabled, the probe was stepped through a fixed
schedule of face-pivot angles to $\pm14^\circ$ and returned, holding $15$~N and
dwelling $3$~s at each angle. Angle tracking held to within $0.002^\circ$ of
each commanded value, off-axis tilt remained below $0.09^\circ$, and lateral
face displacement remained below $0.04$~mm across the sweep, confirming that
the commanded rotation pivots the face rather than translating it and that the
recorded angle is not confounded by lateral coupling.

\emph{Orientation-to-force coupling.} The integral term nulls the force error
at every dwell, so $g_\theta$ is not observable as a force change; it appears
as the change in indentation required to maintain $15$~N, converted through
$K$. Table~\ref{tab:gtheta} reports the result. The coupling is comparatively
small and slowly varying below $6^\circ$, consistent with the cancellation
argument of Section~\ref{sec:control}, and increases by a factor of
approximately three across the lift-off transition predicted above.

\begin{table}[t]
\caption{Orientation-to-force coupling obtained from face displacement at
constant force, $K=2065$~N/m.}
\label{tab:gtheta}
\centering
\footnotesize
\begin{tabular}{ccc}
\toprule
range (deg) & $d\delta/d\theta$ (mm/rad) & $g_\theta$ (N/rad) \\
\midrule
 0--6  & 18.6 &  38 \\
 6--8  & 35.5 &  73 \\
 8--10 & 29.0 &  60 \\
10--12 & 58.9 & 122 \\
12--14 & 21.5 &  44 \\
\bottomrule
\end{tabular}
\end{table}

\emph{Cue sensitivity.} Over the same sweep, the intensity imbalance showed no
statistically resolvable response to tilt within $\pm6^\circ$
($t=-1.8$, $R^2=0.13$), and its full-range regression is dominated by a single
extreme angle. The confidence-depth slope was the only cue exhibiting a
consistent trend, at $-5.7\times10^{-3}$ per degree with $R^2=0.63$ against
angle and no resolvable dependence on elapsed time. Normalizing by the noise
floors of Section~\ref{sec:sensing}, sensitivity per degree per unit noise is
$0.99$ for $I_{\rm slope}$ against $0.27$ for $I_{\rm prox}$, so the
confidence-depth slope more than compensates for the additional noise it
carries. Its advantage is concentrated at the transition of interest:
sensitivity increases from $1.2\times10^{-3}$ per degree below $6^\circ$ to
$2.7\times10^{-2}$ per degree across lift-off, while the intensity imbalance
remains flat. \tbd{confirm the sensitivity and $R^2$ figures in this paragraph
against the cue configuration used for the final sweep}

\emph{Moment channel.} The probe-frame moment about the in-plane axis differed
by approximately $1.5$~Nm between the ascending and descending passes at equal
commanded angle, against a tilt-induced signal of order $0.09$~Nm, and a
quarter of its variance was attributable to elapsed time rather than to angle.
With coupling gel present this hysteresis is attributable to joint-level
friction and transmission effects. The moment channel is therefore not a
viable orientation cue on this platform, which removes the most direct
torque-domain alternative to image-based alignment.


==> sections_v3/06_results.tex <==
\section{Controller Comparison}
\label{sec:results}

\subsection{Protocol}
The controllers of Section~\ref{sec:control} are compared on a cylindrical
gelatin phantom of radius 35 mm,
traversed across the direction of curvature at 5~mm/s with $F_d=15$~N, so that the surface normal in the imaging plane changes
continuously along the path and orientation correction is required rather than
optional. A single controller setting distinguishes the conditions; force
gains, actuator and excursion limits, cue selection, and scanner configuration
are common to all runs and were fixed before collection. The rotation limit and
admissible force band are selected using \eqref{eq:bindcond}:
$\omega_{\max}=0.6$~rad/s and $\Delta F=0.5$~N, held fixed across every
reported condition. Trials are the
experimental unit.

Primary outcomes are the root-mean-square force error and the fraction of the
traverse with $|F_n-F_d|>\Delta F$, which together characterize whether
orientation correction can be applied without violating the contact
specification, and the time-averaged $|I|$, which characterizes whether
alignment is maintained. The secondary outcome is the realized constraint
scale $s$ in P.

Three additional comparisons isolate specific mechanisms. Replacing P's
adaptively-scaled rate limit with a fixed cap at one-third of $\omega_{\max}$
(B2s) tests whether the predictive barrier of \eqref{eq:barrier} does more
than bound the commanded rate. Computing the barrier scale $s$ without
applying it to the commanded rate (Pnc), while leaving delay reconstruction
and coupling prediction active, isolates the barrier's own contribution from
the rest of P. Holding $S$ and $g_\theta$ at their calibrated values
(Table~\ref{tab:gtheta}) rather than estimating them online (P, fixed
parameters) isolates the contribution of adaptation.

\subsection{Results}
Table~\ref{tab:ablation} reports each comparison as a paired trial-level
difference with 95\% confidence intervals; trials within a pair were
collected back-to-back with condition order alternated across pairs to cancel
drift in the phantom and the cue's zero. Force RMSE and out-of-band fraction
did not differentiate any of the orientation-active conditions from one
another -- all five cluster within measurement noise of one another, the
tight $\Delta F=0.5$~N band puts roughly $60\%$ of samples out of band under
every one of them, and the gap that matters is against B1, not between them.

B1 against B2 is unambiguous: applying no orientation correction at all cuts
RMSE by $0.516$~N [$0.467$, $0.565$] and engagement-transient rms error by
$0.322$~N [$0.165$, $0.479$] ($n=5$ pairs). Orientation correction is not
free -- rotating the probe to maintain alignment perturbs contact force
through $g_\theta$ exactly as \eqref{eq:binding} predicts, and B1 pays none of
that cost because it never rotates. The question the remaining rows answer is
not whether correction has a force cost, but whether that cost can be bounded
without giving up alignment.

B2 against P shows the reconstruction-and-prediction architecture reduces
both steady-state RMSE and the engagement transient it otherwise produces by
ringing (force swinging roughly $7\to19.5$~N about the $15$~N target for
$\sim0.5$~s after touchdown). Removing the barrier while leaving estimation
and prediction active (Pnc) reproduces B2's transient almost exactly, and P
against Pnc recovers nearly all of B2 against P's transient benefit while
showing no resolvable steady-state difference -- the barrier accounts for the
transient result and reconstruction accounts for the steady-state result, not
either one for both. The touchdown realignment on this phantom is small
enough that a fixed rate cap could match the barrier by never binding hard
enough to differ, so B2s is compared against P under an imposed $10^\circ$
orientation offset instead, which forces sustained rotation after release and
guarantees the comparison is not made at an operating point where neither
policy is doing real work. There, a fixed rate cap at one-third of nominal
gives significantly worse engagement-transient error than the predictive
barrier ($+0.195$~N [$0.088$,$0.303$] rms, $+0.911$~N [$0.509$,$1.314$]
peak-to-peak contact force, $n=14$ pairs) -- the barrier's advantage over a
naive cap is real once the rotation demand is large enough to expose it.

Holding $S$ and $g_\theta$ at their calibrated values instead of estimating
them online shows no resolvable difference from P on any outcome.
Section~\ref{sec:paramest} addresses why directly: the online estimates moved
only modestly from their calibrated priors over these trials, so there was
little for adaptation to correct on this phantom.

\begin{table}[t]
\caption{Ablation decomposition. Each row is a paired trial-level difference
(condition $A$ minus condition $B$); $^*$ marks a 95\% CI excluding zero. P
denotes the proposed controller (online estimators active). The B2s row uses
an imposed lateral offset rather than the touchdown protocol of
every other row, to guarantee high sustained rotation demand.}
\label{tab:ablation}
\centering
\footnotesize
\setlength{\tabcolsep}{3.0pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{p{0.27\columnwidth}p{0.05\columnwidth}p{0.30\columnwidth}p{0.30\columnwidth}}
\toprule
Comparison ($A-B$) & $n$ & $\Delta$RMSE (N) & $\Delta$rms $|e|$, 1\,s (N) \\
\midrule
B1 $-$ B2                   & 5  & $-0.516$ [$-0.565,-0.467$]$^*$ & $-0.322$ [$-0.479,-0.165$]$^*$ \\
B2 $-$ P                    & 11 & $+0.077$ [$+0.032,+0.122$]$^*$ & $+0.573$ [$+0.402,+0.744$]$^*$ \\
P $-$ Pnc                   & 13 & $-0.020$ [$-0.074,+0.034$]     & $-0.482$ [$-0.624,-0.340$]$^*$ \\
B2 $-$ Pnc                  & 7  & $+0.014$ [$-0.060,+0.088$]     & $-0.147$ [$-0.318,+0.023$] \\
B2s $-$ P (offset) & 14 & --- & $+0.195$ [$+0.088,+0.303$]$^*$ \\
P, fixed $-$ P               & 7  & $-0.019$ [$-0.125,+0.087$]     & $+0.005$ [$-0.148,+0.158$] \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[t]
\centering
\fbox{\parbox[c][1.05in][c]{0.94\columnwidth}{
\centering
\textbf{FIGURE PLACEHOLDER}\\
(a) $g_\theta$ and $I_{\rm slope}$ against known angle, lift-off marked;\\
(b) cue sensitivity per unit noise, three cues;\\
(c) $F_n$ and $I$ along the traverse for B1, B2, and P;\\
(d) realized constraint scale $s$ against predicted excursion.
}}
\caption{Characterization and controller comparison. Metrics are computed from
synchronized $1$~kHz logs; smoothing in representative traces is for display
only.}
\label{fig:results}
\end{figure}

\subsection{Volunteer Feasibility}
A single-subject popliteal scan evaluates whether the frozen controller
operates on living tissue, which introduces spatially varying stiffness,
curvature, and involuntary motion not represented by the phantom. No
independent force reference is available, so this is reported as feasibility
evidence and is not pooled with the phantom statistics.
\tbd{IRB protocol number}

The scan ran for $26.2$~s. Estimated force tracked its setpoint with an RMS
error of $2.64$~N, against $0.98\pm0.06$~N for the same controller on the
phantom, with a peak recorded force of $26.1$~N and a peak error magnitude of
$13.1$~N. Contact was maintained for the whole traverse; the contact flag did
not drop at any point. The time-averaged cue magnitude was $|I|=0.020$, and
the probe reached a maximum angular excursion of $27.4^\circ$ from its
touchdown orientation -- against the $10^\circ$ imposed offset that was
sufficient to separate rate policies on the phantom. The qualitative failure
mode was not loss of contact but failure to null a sustained one-sided
misalignment: the controller held force while the cue, substantially noisier on
living tissue than on homogeneous gelatin, did not drive a consistent
correction. Section~\ref{sec:discussion} takes up what this implies for the
cue rather than for the architecture.
These data do not establish clinical accuracy, anatomical generalization, or
diagnostic image quality.

\subsection{Parameter Estimation}
\label{sec:paramest}
The tilt sweep of Section~\ref{sec:char} calibrates $S$ and $g_\theta$ against
known angle (Table~\ref{tab:gtheta}); the online estimators of
Section~\ref{sec:control} refine these values during operation. Over the
trials collected for the fixed-parameter ablation, the online estimates moved
only modestly from their calibrated priors by trial end: median
$|\Delta S|=4.4\%$ of prior (median $308$ updates), median $|\Delta g_0|=16.6\%$
of prior (median $311$ updates), and $g_1$ moved by $0.008$~N/rad per unit
$I$ from a zero prior. Consistent with this, holding $S$ and $g_\theta$ fixed
at their calibrated values produced no statistically resolvable difference
from online estimation on any outcome (Table~\ref{tab:ablation}, bottom row):
the tilt-sweep calibration was already close to what online estimation
converges to under this phantom's demand. Online adaptation is retained for
surfaces on which that calibration would not hold; Section~\ref{sec:discussion}
discusses the identifiability limits this raises for $g_\theta$ specifically.

==> sections_v3/07_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

The contribution is not the combination of image and force feedback, which is
established~\cite{chatelain2015,jiang2020normal,akbari2021,zakeri2025,piedra2026},
but the explicit treatment of their interaction across the rate gap: what an
orientation command will do to contact force, how much of that the inner loop
will absorb before the next frame arrives, and how much of the observed
alignment error has already been corrected since the frame was captured.

The orientation-to-force coupling is regime-dependent. It is comparatively
small while the face remains fully in contact and increases sharply across the
lift-off transition (Table~\ref{tab:gtheta}). A constant coupling gain would
therefore be conservative in the former regime or insufficient in the latter,
whereas conditioning the gain on the image cue, as in \eqref{eq:gmodel}, tracks
the transition using information already available to the controller.

Whether predicting that coupling alters the commanded correction is determined
in advance by \eqref{eq:bindcond} rather than established empirically. A fast
inner loop attenuates a slow orientation disturbance without assistance, and a
predictive constraint that anticipates an excursion the inner loop would have
rejected contributes nothing. Making the condition explicit identifies which of
rotation limit, force tolerance, and contact gain must change for the
architecture to be consequential, and prevents reporting an advantage at an
operating point where the constraint was never active.

The barrier formulation in \eqref{eq:barrier} addresses a practical
consequence of enforcing the specification as a hard bound. Near the boundary,
a switching constraint maps small fluctuations in the predicted excursion, to
which the image cue contributes directly, into large changes in the commanded
rate. Replacing the switch with a barrier preserves the bound exactly while
making the command a continuous function of the prediction, at the cost of one
additional parameter governing how early the softening begins.

Several limitations qualify these results. The contact-force estimate has no
independent reference during operation and inherits the accuracy bound of
Section~\ref{sec:system}, so all force-tracking results are stated in estimate
space rather than as calibrated force. The confidence map's principal weakness
is that a uniformly anechoic region presents no gradients to the random walk
and may be assigned high confidence; the resulting cue therefore reports
asymmetry reliably but is not a contact detector. The online estimator for
$g_\theta$ regresses force residuals on rotation and does not observe surface
elevation, so any force variation arising from the traversed geometry or from
tissue motion is attributed to rotation; this limits identifiability on curved
paths and on living tissue, and motivates the fixed-parameter configuration
reported alongside the adaptive one. On the homogeneous phantom used here, the
fixed-parameter ablation (Section~\ref{sec:paramest}) found no resolvable
difference from online estimation, and the online estimates themselves moved
little from their calibrated priors over a trial -- consistent with, not
contradicting, the identifiability concern: adaptation had little to correct
because the tilt-sweep calibration already held. Surfaces or tissue that
violate that calibration, which the estimator's own limited identifiability
leaves unaddressed, are exactly where a difference would be expected to
appear, and this evaluation does not reach them.

The volunteer scan makes the cue, rather than the architecture, the binding
limitation on living tissue. Force was regulated and contact was maintained
for the full traverse, but the cue was substantially noisier than on
homogeneous gelatin and the controller did not reliably null a sustained
one-sided misalignment, reaching an angular excursion well beyond anything the
phantom protocol demanded. Because the cue enters \eqref{eq:imglaw} directly
and without smoothing -- deliberately, since a filter would introduce lag that
the delay reconstruction of \eqref{eq:recon} does not model -- cue noise
converts into commanded rotation with no intervening attenuation. The
excursion limit bounds the consequence but does not address the cause. A cue
conditioned on tissue rather than tuned on a phantom, or an explicit detector
for large-area decoupling of the kind Section~\ref{sec:control} notes the
asymmetry cue cannot provide, is the natural next step and is not attempted
here. Finally, characterization is confined to homogeneous gelatin, and the
volunteer scan is a single-subject feasibility test that establishes neither
clinical safety nor anatomical generalization.

==> sections_v3/08_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We presented a dual-rate orientation controller for robotic ultrasound in which
the slow image-guided loop reconstructs the alignment error to the current
instant from the capture timestamp of the frame it was computed from, predicts
the force excursion that a candidate correction would produce using an
orientation-to-force coupling conditioned on the image cue, and credits the
fast force loop with the portion of that disturbance it will reject within the
frame interval, so that the correction is limited only to the extent the
contact specification requires. The controller operates without a force/torque
sensor, with contact force estimated from joint torques.

Supporting identification against known probe angle yields the
orientation-to-force coupling, which is comparatively small while the probe
face remains fully in contact and increases by approximately a factor of three
across lift-off, and establishes a confidence-depth slope as the most
favorable of the evaluated image cues in sensitivity per unit noise. We further
give the explicit condition under which the predictive constraint modifies the
commanded correction, and select the operating point accordingly. On the
phantom, orientation correction carries a measurable force cost relative to
holding orientation fixed, and the proposed controller recovers part of that
cost against a newest-frame baseline, with the predictive barrier accounting
for the engagement transient and delay reconstruction for the steady-state
error; a single-subject popliteal scan maintained contact throughout but did
not reliably null sustained misalignment, locating the limitation on living
tissue in the image cue rather than in the control architecture.
Claims are restricted to the tested phantom, force, angle, and timing ranges.

\section*{Acknowledgment}
The authors acknowledge support from The University of Alabama faculty startup
fund and the Alabama Transportation Institute. This work was also supported by
the U.S. Department of Transportation University Transportation Centers Program
through CR2C2, Grant No.~69A3552348304.


==> sections_v4/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Brightness mode (B-mode) ultrasound provides real-time, radiation-free imaging at comparatively low cost, but its image quality depends strongly on how the probe interacts with tissue. A sonographer continuously coordinates probe position, orientation, and contact force while responding to surface geometry, tissue compliance, and the image itself, so robotic ultrasound is a coupled sensing-and-control problem rather than a trajectory-following task. Reviews accordingly identify scan-path generation, probe--tissue force regulation, and image-quality or orientation optimization as the central components of autonomous systems \cite{li2021overview,salcudean2022,jiang2023review}, and recent surveys note that orientation-related interaction forces are often simplified and that real-time image feedback is still rarely integrated into online scan optimization \cite{bi2024,munir2025,han2025clinical}.

Image features extracted directly from ultrasound can close the robot-positioning loop \cite{abolmaesumi2002}, and visual servoing on ultrasound confidence has been used to improve acoustic coupling and probe orientation \cite{chatelain2015}. Interaction-force information has been used to estimate the local surface normal and regulate orientation \cite{jiang2020normal,jiang2021force,ma2022asee}, explicit force/moment control improves interaction under heterogeneous contact \cite{piedra2026}, ultrasound feedback has enabled autonomous screening of tubular structures \cite{jiang2022tubular}, and image-quality estimates have been used to adapt the commanded force \cite{akbari2021,zakeri2025}. Image and force sensing are therefore established as complementary, and combining them is no longer, by itself, a contribution to control. Learning-based methods have extended autonomy to navigation, compliant scanning, and complete clinical workflows \cite{hase2020,ning2021rl,jiang2025ultrabot}, including policies trained under explicit force constraints \cite{duan2025safe}; this work instead keeps a physically structured force loop and uses the image only as a measured cue.

A control issue that is less explicitly addressed is the multirate dynamic coupling between force regulation and image-guided probe correction. Robot state and wrench estimates update at high rates, whereas B-mode images are acquired, transferred, and processed at much lower rates and with non-negligible latency; image-based force adjustment, for example, has been run with an image loop slower than the underlying robot loop \cite{akbari2021}. The difficulty is more fundamental than asynchronous sensing alone. An orientation correction computed from an image changes probe indentation, the contact moment, and consequently the normal force before a new image becomes available. Conversely, a fast force regulator reacts to the normal displacement induced by the orientation update and can partially oppose the intended correction. Tissue stiffness, local curvature, and uncertainty in image sensitivity further modify this bidirectional interaction. Dual-loop approaches have demonstrated image-dependent force adaptation and robust force tracking \cite{zakeri2025}, Li \emph{et al.}~\cite{li2026trajectory} incorporate trajectory-dependent feedforward and delay compensation for contact-force tracking, and Qian \emph{et al.}~\cite{qian2026symmetry} combine image guidance with biomechanics-informed force measurement. These approaches do not, however, treat the image-guided orientation loop and the high-rate force loop as a delayed multirate system whose cross-coupling is predicted and used in the controller.

This paper treats that coupling as the control problem. We propose a dual-rate orientation controller in which the slow image-guided loop accounts for both its own latency and its effect on the fast contact loop: the alignment error is reconstructed to the present instant from the frame's capture timestamp; the force excursion that a candidate correction would produce is predicted from a conservative bound on the rotation-to-force gain; and the prediction credits the fast loop with the part of that excursion it will reject before the next frame arrives. The last term separates the method from a one-step safety filter, which must assume the excursion persists and therefore throttles the correction more than necessary.

The controller runs on a platform with \emph{no force/torque sensor}; contact force is estimated from joint torques. This raises the force noise floor and introduces model-dependent bias, so the force margins the controller must respect are small relative to the estimate's own error. The contributions are:

\vspace{-0.5mm}
\begin{enumerate}
    \item a dual-rate orientation controller combining timestamp-based delay reconstruction with a force-excursion constraint that uses a conservative rotation-to-force gain bound and credits the fast force loop's rejection over the frame interval; and

    \item a hardware evaluation on a curved phantom against force-only, newest-frame, and fixed-rate-cap baselines, with ablations isolating the constraint, the fast-loop credit, and online sensitivity estimation, together with a model-free measurement of the rotation-to-force gain and a volunteer popliteal scan.
\end{enumerate}


==> sections_v4/02_system.tex <==
\section{System and Sensorless Force Estimation}
\label{sec:system}

\subsection{Platform}
The platform (Fig.~\ref{fig:setup}) is a Kinova Gen3 six-degree-of-freedom manipulator carrying a Telemed Artus linear probe in a rigid printed holder. No force/torque sensor is present; the contact wrench is estimated from the torque sensors in each actuator. This removes the cost, cabling, and sterilization burden of a wrist-mounted transducer at the expense of a higher noise floor and a model-dependent bias.

The arm is commanded in joint position at $f_f=1$~kHz through the manufacturer's low-level cyclic interface. A Cartesian velocity command $v_c\in\mathbb R^{6}$ is mapped to joint rates through a damped least-squares inverse $J^{\dagger}$ of the geometric Jacobian $J(q)\in\mathbb R^{6\times6}$ and integrated to the streamed position command,
\begin{equation}
\dot q_c=J^{\dagger}(q)\,v_c,\qquad
q_c^{k+1}=q_c^{k}+\dot q_c\,\Delta t_f,
\label{eq:intcmd}
\end{equation}
with $q\in\mathbb R^{6}$ the measured joint coordinates and $\Delta t_f=1/f_f$. B-mode frames are captured from the scanner display at $f_I=30$~Hz, and each is tagged with its capture time. The scanner's internal acquisition-to-display delay was not resolved and is not compensated.

\begin{figure}[t]
\centering
\fbox{\parbox[c][1.55in][c]{0.94\columnwidth}{\centering
\textbf{FIGURE PLACEHOLDER}\\ photograph of the setup: arm, probe and holder, cylindrical phantom, scanner display}}
\caption{Experimental setup. \tbd{photo and callouts}}
\label{fig:setup}
\end{figure}

\subsection{Wrench Estimation from Joint Torques}
With $\tau_m\in\mathbb R^{6}$ the measured joint torques and $h_c\in\mathbb R^{6}$ the contact wrench at the tool, the rigid-body model is
\begin{equation}
M(q)\ddot q+C(q,\dot q)\dot q+\tau_g(q)+\tau_r=\tau_m+J^{\!\top}(q)\,h_c ,
\label{eq:dyn}
\end{equation}
where $\tau_g$ is the gravity torque and $\tau_r$ a joint-level residual. The inertial and Coriolis terms are omitted: the scan feed is $5$~mm/s, and, evaluated post hoc from the logged trajectories, the omitted terms contribute at most \result{X}~N to the regulated force at rotation onset and \result{Y}~N during the traverse. Including them online would require differentiating the actuators' velocity feedback, itself a numerical derivative, which amplifies noise. The gravity torque is computed by a quasi-static recursive Newton--Euler pass \cite{featherstone2008} with link parameters from the manufacturer's model, the last link's mass and center of mass updated for the probe and holder, and the gravity vector corrected for the base mounting tilt.

The residual $\tau_r$ depends on joint position and on the direction of recent motion. It is modeled per joint by two branches, each a constant plus low-frequency harmonics of joint angle (periods of $45$--$290^\circ$) identified offline from free-space pose sweeps. The weight between branches evolves as a single stop operator of width $1^\circ$ \cite{brokate1996}, so the model blends linearly between branches over the first degree of travel after a reversal; it is a low-order model with no minor-loop memory. The estimated contact wrench is
\begin{equation}
\hat h_c=\bigl(J^{\!\top}(q)\bigr)^{\!+}
\bigl(\bar\tau_m-\tau_g(q)-\hat\tau_r(q)\bigr)-h_0 ,
\label{eq:wrench}
\end{equation}
where $\bar\tau_m$ is $\tau_m$ after a per-joint second-order Butterworth filter with a $25$~Hz cutoff, $(\cdot)^{+}$ denotes the pseudoinverse, $\hat\tau_r$ is the residual model, and $h_0\in\mathbb R^{6}$ is a free-space tare acquired while the arm holds position immediately before contact. Because $h_0$ absorbs whatever residual the model leaves at that pose, it is preceded by a conditioning motion that walks each joint against and then along its press direction, so the tare is taken on the same branch that the subsequent press will traverse.

The regulated variable is the beam-axis component of the estimated contact force in a probe frame whose origin is the acoustic face,
\begin{equation}
F_n=-\,e_3^{\!\top}\,{}^{P}\!R_B\,\hat F_c ,
\label{eq:fn}
\end{equation}
where $\hat F_c\in\mathbb R^{3}$ is the force part of $\hat h_c$, ${}^{P}\!R_B\in SO(3)$ the base-to-probe rotation, and $e_3\in\mathbb R^{3}$ selects the beam axis, which points out of the face, so compression is positive.

\subsection{Achievable Accuracy}
Since \eqref{eq:wrench} has no independent force reference during operation, its accuracy bounds every downstream claim, and all force results are stated in estimate space. Static loading against a reference scale over $5$--$20$~N gives an RMS error of \result{A}~N with the residual model and \result{B}~N without it. The residual model mainly matters after a joint reversal, where it reduces the error from \result{C}~N to \result{D}~N RMS. These figures bound the estimate rather than calibrate it.


==> sections_v4/03_sensing.tex <==
\section{Orientation Sensing from Ultrasound}
\label{sec:sensing}

When the probe deviates from the local surface normal, acoustic coupling degrades on one side of the aperture and image quality falls off from the transducer face downward on that side. We quantify this asymmetry with a scalar cue $I$, dimensionless, with $I=0$ corresponding to a laterally symmetric image.

The cue is computed from the ultrasound confidence map of Karamalis \emph{et al.}~\cite{karamalis2012}, which assigns to each pixel the probability that a random walker released there reaches the transducer before the far field, with edge weights derived from intensity gradients under an attenuation model. Writing $c(r,\kappa)\in[0,1]$ for the confidence at row $r$ and column $\kappa$, the map is obtained by solving a sparse Dirichlet problem on the pixel graph, here at $96\times96$ on a fixed crop of the displayed image (which includes the scanner's on-screen markings) by direct factorization with the symbolic analysis performed once. The per-frame cost on the experimental hardware, including crop, resize, solve, and feature extraction, was \result{mean $\pm$ sd}~ms, against the $33$~ms frame interval. Each result is tagged with the capture time of the frame from which it was computed.

The cue uses the depth at which confidence falls below a threshold $c_{\rm th}$,
\begin{equation}
d(\kappa)=\frac{1}{N_r-1}\min\{\,r:\;c(r,\kappa)<c_{\rm th}\,\},
\label{eq:cdepth}
\end{equation}
with $N_r$ the number of rows, and takes its least-squares slope against normalized lateral position $x_\kappa\in[-1,1]$, negated so that a more confident left side gives a positive value:
\begin{equation}
I=-\,\Bigl(\textstyle\sum_\kappa x_\kappa d(\kappa)\Bigr)
\Bigl/\Bigl(\textstyle\sum_\kappa x_\kappa^{2}\Bigr).
\label{eq:cslope}
\end{equation}
Because \eqref{eq:cslope} depends on the depth at which the reliable region ends rather than on the confidence level itself, a spatially uniform change in gain or in overall confidence leaves it unchanged. Map parameters were selected offline on recorded scans: $\alpha=2.0$, $\beta=10.0$, $\gamma=0.05$, and $c_{\rm th}=0.5$.

The cue used for control, $I_f$, is $I$ passed through a second-order Butterworth low-pass filter with a $10$~Hz cutoff, stepped at $1$~kHz on the most recent frame value. Its group delay near DC, $\tau_f=\sqrt2/(2\pi\cdot10~\mathrm{Hz})=22.5$~ms, is compensated in the delay reconstruction of Section~\ref{sec:control}.

The cue presupposes that most of the aperture is coupled. If contact is lost across a large fraction of the face, $I$ remains well defined but no longer reports misalignment. This is a limitation of the cue rather than a condition the controller detects; the excursion limit of Section~\ref{sec:control} bounds how far a misreported cue can drive the probe.


==> sections_v4/04_control.tex <==
\section{Dual-Rate Control}
\label{sec:control}
\begin{figure*}[t]
  \centering
  \input{figures/architecture_diagram}
  \caption{Dual-rate control architecture. The $30$~Hz image loop reconstructs the cue to the present instant and scales the orientation command through the force-excursion constraint; the $1$~kHz force loop regulates the estimated contact force.}
  \label{fig:control_architecture}
\end{figure*}

\subsection{Fast Force Loop}
The force loop regulates $F_n$ to a constant reference $F_d$ by commanding beam-axis velocity at $1$~kHz,
\begin{equation}
v_n=K_p e_F-K_d\dot F_n,
\qquad e_F=F_d-F_n,
\label{eq:pd}
\end{equation}
with $v_n$ saturated at $0.04$~m/s and the derivative taken on the measurement. No integral term is used: the plant integrates the velocity command, so the loop already rejects constant disturbances. Gains were tuned at the operating force ($K_p=6.25\times10^{-3}$~m\,N$^{-1}$s$^{-1}$, $K_d=6.25\times10^{-5}$~m\,N$^{-1}$) and held fixed across every reported condition.

Locally, the contact obeys $\dot F_n=K v_n+g_\theta\,\omega$, where $K$ is the contact stiffness, $\omega$ the probe's rotation rate in the image plane, and $g_\theta$ the rotation-to-force gain defined below. With \eqref{eq:pd}, the force error then evolves as
\begin{equation}
\dot e_F=-a\,e_F-g'\omega,
\label{eq:arate}
\end{equation}
with $a=KK_p/(1+KK_d)$ the fast loop's disturbance-rejection rate and $g'=g_\theta/(1+KK_d)$. $K$ is identified once per contact from the loading ramp, by a least-squares fit of $F_n$ against face depth along the beam axis (from forward kinematics, filtered like the torques) over the samples between $0.4F_d$ and touchdown; a fit with fewer than $100$ samples or $R^2<0.9$ is rejected in favor of a prior. The ramp precedes the scan feed, so surface elevation does not enter the fit. On the phantom of Section~\ref{sec:char}, $K=$~\result{K}~N/m, giving $a=$~\result{a}~s$^{-1}$.

\subsection{Orientation Channel}
The orientation loop rotates the probe about the in-plane axis of its face, changing its tilt $\theta$ in the image plane (measured from the touchdown orientation), so as to drive the cue to zero,
\begin{equation}
\omega=-K_I\,\sigma\,I,\qquad
\sigma=\operatorname{sign}\!\left(S\right),
\label{eq:imglaw}
\end{equation}
with cue gain $K_I>0$ and $\omega$ saturated at $\omega_{\max}$. The command is mapped to the Jacobian's reference point so that the face pivots in place rather than translating. Net angular excursion from the touchdown orientation is limited to $0.55$~rad; beyond the limit only rotation back toward the touchdown orientation is permitted, so the limit bounds departure without preventing recovery.

The law \eqref{eq:imglaw} acts directly on the cue and needs no conversion to angle. Two model quantities are nevertheless required by the terms below: the cue sensitivity $S=\partial I/\partial\theta$, which converts elapsed rotation into an equivalent change in the cue, and the rotation-to-force gain $g_\theta=\partial F_n/\partial\theta$ at fixed face position, which converts a candidate rotation into a force excursion. $S$ is estimated online by recursive least squares with forgetting ($\lambda=0.99$), with its sign fixed from calibration and updates gated on appreciable rotation. $g_\theta$ is not estimated online: replaying the estimator on earlier phantom logs showed it is not identifiable from the controller's own rotations. It is instead held at a conservative bound $\bar g=40$~N/rad, above every value measured in Section~\ref{sec:char}.

\subsection{Compared Controllers}
All controllers share the force loop, the rotation and excursion limits, and the cue.

\textbf{B1} applies no orientation correction, $\omega\equiv0$.

\textbf{B2} applies \eqref{eq:imglaw} to the most recent filtered cue $I_f$, with no delay reconstruction and no force constraint.

\textbf{P} adds two terms. The first is \emph{delay reconstruction}. The cue was measured at capture time $t^c$ and the probe has rotated since, so the controller acts on
\begin{equation}
\hat I(t)=I_f(t)+S\bigl(\theta(t)-\theta(t^c-\tau_f)\bigr),
\label{eq:recon}
\end{equation}
with $\theta$ read from a $1$~kHz history buffer; the shift by $\tau_f$ compensates the filter's group delay. The second is a \emph{force-excursion constraint with fast-loop credit}. At each new frame the controller simulates, over a horizon $T_h=100$~ms that covers the interval until the next frame,
\begin{equation}
\dot\varepsilon=-a\,\varepsilon+\bar g'\omega,\quad
\dot{\hat I}=S\,\omega,\quad
\omega=s\,\operatorname{sat}\bigl(-K_I\sigma\hat I\bigr),
\label{eq:predsim}
\end{equation}
from $\varepsilon(0)=0$, where $\bar g'=\bar g/(1+KK_d)$ and $\varepsilon$ is the part of $F_n-F_d$ caused by the rotation. Because the loop is linear, the current force error evolves the same way with or without rotation and cancels, so the constraint acts only on the excursion the rotation adds; removing the existing error is the force loop's task. The second equation lets the commanded rate fall as the cue is nulled within the horizon. With $u(s)=\max_{[0,T_h]}|\varepsilon|/\Delta F$, the scale on the commanded rate is
\begin{equation}
s=\arg\min_{s\in[0,1]}\;(1-s)^2-\mu\log\!\bigl(1-u(s)^2\bigr),
\label{eq:barrier}
\end{equation}
held until the next frame, with $\mu=0.05$. The first term is the cost of withholding correction: zero at full correction and largest at none. The second is a logarithmic barrier on the excursion budget $\Delta F$: negligible while the predicted excursion is small, so $s\to1$ when the correction is harmless, and unbounded as the prediction approaches $\Delta F$, so no minimizer can exceed it. The scale therefore varies continuously with the prediction rather than switching at the boundary, which matters because the prediction inherits the frame-to-frame variability of the cue.

The term $-a\varepsilon$ is what distinguishes P from a one-step constraint. A one-step constraint assumes the excursion accumulates unopposed, $\bar g\,\omega T_h$ over the horizon, whereas P credits the fast loop, which limits it to $(\bar g'\omega/a)(1-e^{-aT_h})$, so the correction is throttled less. The ablations change one setting each. \textbf{P\textsubscript{nb}} computes $s$ but does not apply it, isolating the constraint from reconstruction. \textbf{P\textsubscript{fix}} holds $S$ at its calibrated value. \textbf{P\textsubscript{1s}} is P\textsubscript{fix} with $a=0$ (and $\bar g'=\bar g$), the one-step constraint. \textbf{B2\textsubscript{cap}} is B2 with $\omega_{\max}$ fixed at one third of nominal, testing whether the constraint does more than a fixed rate cap.

\subsection{Activity of the Constraint}
At full rate, the constraint modifies the command only if the predicted excursion exceeds the budget,
\begin{equation}
\frac{\bar g'\,\omega_{\max}}{a}\bigl(1-e^{-aT_h}\bigr)\;\gtrsim\;\Delta F .
\label{eq:bindcond}
\end{equation}
The rotation limit $\omega_{\max}$ is the worst case, and at this operating point also the actual one, since the rate saturates immediately after touchdown. Condition \eqref{eq:bindcond} can be checked before experiments: a fast force loop, a slow rotation limit, or a wide budget each make the constraint inactive, in which case P reduces to B2 with reconstruction, while compliant contacts, reduced force gains, and lower-bandwidth force loops enlarge the regime in which it acts. We use $\omega_{\max}=0.6$~rad/s and $\Delta F=0.5$~N, for which \eqref{eq:bindcond} holds with $\bar g$ (predicted excursion \result{E}~N at full rate), and report the realized scale $s$ so that the comparison is not made at an operating point where the constraint never acts. $\Delta F$ is a budget on the rotation-induced excursion, not a force-tracking band.


==> sections_v4/05_characterization.tex <==
\section{Characterization}
\label{sec:char}

All phantom experiments used a cylindrical gelatin phantom of radius $35$~mm, prepared from water, gelatin, and cornstarch (a speckle agent) in an $80\!:\!10\!:\!1$ weight ratio, with coupling gel at the interface. Scanner gain, dynamic range, time-gain compensation, speckle reduction, and adaptive gain were fixed for all runs, since the cue is comparable only within a fixed display configuration. Characterization was performed from the same taught start pose as the controller comparison of Section~\ref{sec:results}.

\subsection{Contact Stiffness}
Over the loading ramps of all phantom runs, the per-contact fit of Section~\ref{sec:control} gave $K=$~\result{median [range]}~N/m with $R^2$ of \result{range}; \result{n} of \result{N} fits were rejected in favor of the prior.

\subsection{Tilt Sweep}
With the orientation loop disabled, the probe was stepped through face-pivot angles out to $\pm12^\circ$ and back while holding $15$~N, dwelling $3$~s at each angle. The force loop returns $F_n$ to $F_d$ at every dwell, so $g_\theta$ is not observable as a force change; it appears as the depth change needed to maintain $15$~N. With $x$ the face depth along the touchdown beam axis, $y=F_n-Kx$ is the force the tilt would have added at fixed depth, and $g_\theta=\mathrm{d}y/\mathrm{d}\theta$. No contact model is assumed: $g_\theta$ is estimated as the local slope of $y$ within fixed $4^\circ$ angle bands, after removing a slow drift in $y$ over the sweep (gel relaxation) that the ascending and descending passes separate.

\emph{Rotation-to-force gain.} Because the surface is symmetric about its normal, $y$ is even about the tilt $\theta_n$ at which the face is normal to the surface, so $g_\theta$ vanishes there and changes sign across it. The measured $y$ had its vertex at $\theta_n=$~\result{$\theta_n$ [CI]}$^\circ$, and $|g_\theta|$ remained at or below \result{max band value}~N/rad over the swept range (largest 95\% bound \result{?}~N/rad), \result{ratio}$\times$ below $\bar g$. \tbd{If a band shows a kink consistent with an edge losing contact, state its angle here.}

\emph{Cue sensitivity.} Over the same dwells, the cue varied with tilt at $S=$~\result{S [CI]}~rad$^{-1}$ ($R^2=$~\result{?}), which sets the calibrated value used by P\textsubscript{fix} and the prior for online estimation. Its zero lay at \result{?}$^\circ$ from upright. \tbd{Compare with $\theta_n$: if $\theta_n\approx0$, the cue's zero is offset from the true normal (a cue bias, e.g., from the crop); if $\theta_n$ lies near the cue's zero, the upright start pose was not normal to the surface and the cue reports it correctly.} \tbd{If the banded slopes show the cue flat near normal and steep further out, state that the cue responds mainly to loss of coupling at one edge.}

\subsection{Latency}
The control signal's age at use, from frame capture to the controller, had a median of \result{?}~ms (95th percentile \result{?}~ms), the confidence map running one frame behind the newest capture. The additional acquisition-to-display delay internal to the scanner was not resolved by a lag scan against known angle (\result{?}~ms, 95\% CI \result{?}).


==> sections_v4/06_results.tex <==
\section{Controller Comparison}
\label{sec:results}

\subsection{Protocol}
The controllers of Section~\ref{sec:control} were compared on the phantom of Section~\ref{sec:char}, traversed along its axis for $150$~mm at $5$~mm/s with $F_d=15$~N and image-based lateral centering active. The surface normal is constant along this path; the orientation demand arises at engagement, because every run starts from the same taught upright pose and the cue's zero lies \result{?}$^\circ$ from it, so the orientation loop rotates the probe by about that amount immediately after touchdown. All parameters, including $\omega_{\max}=0.6$~rad/s, $\Delta F=0.5$~N, $\bar g=40$~N/rad, the force gains, the cue, and the scanner configuration, were fixed before collection. Conditions were collected in interleaved ABBA blocks of \result{10} pairs, and each trial is one experimental unit.

The outcomes are the RMS force error over the first second after touchdown, $E_1$, which captures the engagement transient; the RMS force error over the full traverse, $E$; the time-averaged cue magnitude $\overline{|I|}$, which measures whether alignment is achieved; and, for the P family, the realized minimum scale $s_{\min}$ in the first $0.5$~s. Table~\ref{tab:ablation} reports paired differences.

\begin{table}[t]
\caption{Paired differences between conditions (A $-$ B), mean [95\% CI].}
\label{tab:ablation}
\centering
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lcccc}
\toprule
A $-$ B & $n$ & $\Delta E_1$ (N) & $\Delta E$ (N) & $\Delta\overline{|I|}$ \\
\midrule
B1 $-$ B2                                 & \result{?} & \result{?} & \result{?} & \result{?} \\
B2 $-$ P                                  & \result{?} & \result{?} & \result{?} & \result{?} \\
P\textsubscript{nb} $-$ P                 & \result{?} & \result{?} & \result{?} & \result{?} \\
B2 $-$ P\textsubscript{nb}                & \result{?} & \result{?} & \result{?} & \result{?} \\
B2\textsubscript{cap} $-$ P               & \result{?} & \result{?} & \result{?} & \result{?} \\
P\textsubscript{1s} $-$ P\textsubscript{fix} & \result{?} & \result{?} & \result{?} & \result{?} \\
P\textsubscript{fix} $-$ P                & \result{?} & \result{?} & \result{?} & \result{?} \\
\bottomrule
\end{tabular}\\[2pt]
\raggedright\scriptsize $^*$95\% CI excludes zero.
\end{table}

\subsection{Results}
\tbd{All statements in this subsection are to be verified against the re-collected data; the structure follows the expected outcomes.}

\emph{Cost of correction.} B1 never rotates and so pays no force cost for alignment; against B2, it changes $E_1$ by \result{?} and $E$ by \result{?}, while leaving the cue uncorrected ($\Delta\overline{|I|}=$~\result{?}). Orientation correction is not free: rotating the probe perturbs contact force through $g_\theta$. The remaining rows ask whether that cost can be bounded without giving up alignment.

\emph{Engagement transient.} Under B2 the probe rotates at the full rate from touchdown, and the estimated force swings between \result{?} and \result{?}~N about the $15$~N target over roughly \result{?}~s (Fig.~\ref{fig:force}). P reduces $E_1$ by \result{?} relative to B2, with a realized $s_{\min}$ of \result{?} at engagement. Removing the constraint while keeping reconstruction and online estimation (P\textsubscript{nb}) reproduces B2's transient, so the constraint accounts for the transient result; reconstruction alone (B2 $-$ P\textsubscript{nb}) accounts for \result{the steady-state difference / no resolvable difference}. The transient reduction is reported empirically: the quasi-static prediction in \eqref{eq:predsim} does not describe the engagement swing itself, and the constraint limits it through the conservatism of $\bar g$.

\emph{Constraint versus a fixed cap.} A fixed rate cap at one third of nominal (B2\textsubscript{cap}) changes $E_1$ by \result{?} relative to P, with $\Delta\overline{|I|}=$~\result{?}. Because every run rotates at the full rate at engagement, both the cap and the constraint act on the same demand, so the comparison is not made at an operating point where neither limit binds.

\emph{Fast-loop credit and adaptation.} Crediting the fast loop (P\textsubscript{fix} against P\textsubscript{1s}) raises $s_{\min}$ from \result{?} to \result{?} and changes $E_1$ by \result{?} and $\overline{|I|}$ by \result{?}. Holding $S$ at its calibrated value (P\textsubscript{fix}) changes no outcome by more than \result{?}.

\begin{figure}[t]
\centering
\fbox{\parbox[c][1.55in][c]{0.94\columnwidth}{\centering
\textbf{FIGURE PLACEHOLDER}\\ $F_n$, first 1.5~s after touchdown: median and interquartile range across trials for B2, P, B2\textsubscript{cap}; $\pm\Delta F$ shaded}}
\caption{Estimated contact force at engagement. \tbd{final figure}}
\label{fig:force}
\end{figure}

\begin{figure}[t]
\centering
\fbox{\parbox[c][1.55in][c]{0.94\columnwidth}{\centering
\textbf{FIGURE PLACEHOLDER}\\ cue $I$ along the traverse: median and interquartile range across trials for B1, B2, P}}
\caption{Alignment cue along the traverse. \tbd{final figure}}
\label{fig:cue}
\end{figure}

\subsection{Volunteer Feasibility}
A single-subject popliteal scan tests whether the frozen controllers operate on living tissue, which adds spatially varying stiffness and curvature and subject motion (arterial pulsation, muscle activity, and limb drift) not represented by the phantom. It is reported as feasibility evidence and is not pooled with the phantom statistics. \tbd{IRB protocol number}

P and B2 were each run \result{n} times. Under P, the estimated force tracked its setpoint with an RMS error of \result{?}~N (B2: \result{?}~N), with a peak error magnitude of \result{?}~N; contact was maintained for \result{?} of the traverse, and $\overline{|I|}$ was \result{?} (B2: \result{?}). \tbd{If the new data again shows a sustained one-sided misalignment that the controller does not null, describe it as the confidence map's insufficiency under partial coupling; otherwise remove.} These data do not establish clinical accuracy, anatomical generalization, or diagnostic image quality.


==> sections_v4/07_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

The contribution is not the combination of image and force feedback, which is established~\cite{chatelain2015,jiang2020normal,akbari2021,zakeri2025,piedra2026}, but the explicit treatment of their interaction across the rate gap: what an orientation command will do to contact force, how much of that the force loop will absorb before the next frame arrives, and how much of the observed alignment error has already been corrected since the frame was captured.

The rotation-to-force gain depends on surface geometry and contact state. On the cylindrical phantom it vanishes at the normal and grows with tilt (Section~\ref{sec:char}), and it was not identifiable online from the controller's own rotations. The controller therefore uses a conservative bound rather than a model. A bound is redundant at worst where the true gain is small, costing some alignment speed, but it cannot understate the force a rotation adds.

That conservatism is also why the constraint is active here. With the measured gain in place of $\bar g$, \eqref{eq:bindcond} would not hold at this operating point, and the constraint would rarely modify the command \tbd{verify with the measured gain}. The quasi-static prediction also does not describe the dynamic force swing at engagement; the constraint limits that swing because $\bar g$ overstates the gain, not because the swing is predicted. The transient result is accordingly reported as an empirical outcome, not a guarantee.

Several limitations qualify these results. The contact-force estimate has no independent reference during operation and inherits the accuracy bound of Section~\ref{sec:system}, so all force results are stated in estimate space rather than as calibrated force. The confidence map's principal weakness is that a uniformly anechoic region presents no gradients to the random walk and may be assigned high confidence, so the cue reports asymmetry reliably but is not a contact detector. \tbd{If large-area decoupling recurs in the new data, add it here as a second weakness.} Surfaces or tissue on which the true gain approaches or exceeds $\bar g$, such as stiffer tissue or sharper curvature, are exactly where the bound would need to change, and this evaluation does not reach them.

The volunteer scan \tbd{(verify against the new data)} makes the cue, rather than the architecture, the binding limitation on living tissue. The cue is low-pass filtered and the filter's group delay is compensated in \eqref{eq:recon}, but residual cue noise on tissue still converts directly into commanded rotation, and the excursion limit bounds the consequence without addressing the cause. A cue conditioned on tissue rather than tuned on a phantom, or an explicit detector for large-area decoupling of the kind Section~\ref{sec:sensing} notes the cue cannot provide, is the natural next step and is not attempted here. Finally, characterization is confined to homogeneous gelatin, and the volunteer scan is a single-subject feasibility test that establishes neither clinical safety nor anatomical generalization.


==> sections_v4/08_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We presented a dual-rate orientation controller for robotic ultrasound in which the slow image-guided loop reconstructs the alignment error to the current instant from the capture timestamp of the frame it was computed from, predicts the force excursion that a candidate correction would produce using a conservative bound on the rotation-to-force gain, and credits the fast force loop with the portion of that excursion it will reject within the frame interval, so that the correction is limited only to the extent the contact specification requires. The controller operates without a force/torque sensor, with contact force estimated from joint torques.

A model-free tilt sweep on a curved phantom showed the rotation-to-force gain vanishing at the surface normal and remaining at or below \result{?}~N/rad over the swept range, below the bound used by the controller, and the operating point was chosen so that the constraint is active under that bound. On the phantom, orientation correction carries a measurable force cost relative to holding orientation fixed, and \result{summary of B2 $-$ P and the ablations}. A single-subject popliteal scan \result{summary}. Claims are restricted to the tested phantom and force range.

\section*{Acknowledgment}
The authors acknowledge support from The University of Alabama faculty startup fund and the Alabama Transportation Institute. This work was also supported by the U.S. Department of Transportation University Transportation Centers Program through CR2C2, Grant No.~69A3552348304. Generative AI was used in preparing this manuscript. \tbd{AI Tool Used} was used to generate the initial outline and early draft structure. Claude (Anthropic) was used to draft text in Sections I–VIII from the authors' notes, technical decisions, and source code, and to edit the manuscript for clarity and grammar; [Sections ex.(I, VII, and VIII)] were subsequently rewritten by the authors. [The source for Fig. 2 was generated with AI assistance.] All technical content was verified by the authors.
